Dark Bursts in the Swift Era: The Palomar 60 inch-Swift Early Optical Afterglow Catalog

We present multi-color optical observations of long-duration gamma-ray bursts (GRBs) made over a three year period with the robotic Palomar 60 inch telescope (P60). Our sample consists of all 29 events discovered by Swift for which P60 began observations less than one hour after the burst trigger. We were able to recover 80% of the optical afterglows from this prompt sample, and we attribute this high efficiency to our red coverage. Like Melandri et al. (2008), we find that a significant fraction (~ 50%) of Swift events show a suppression of the optical flux with regards to the X-ray emission (so-called "dark" bursts). Our multi-color photometry demonstrates this is likely due in large part to extinction in the host galaxy. We argue that previous studies, by selecting only the brightest and best-sampled optical afterglows, have significantly underestimated the amount of dust present in typical GRB environments.

==> tab1.tex <==
\ProvidesFile{p60catalog.tab.tex}

\begin{deluxetable}{crrrrr}
  \tabletypesize{\footnotesize}
  \tablecaption{P60-\Swift\ Early Optical Afterglow Catalog}
  \tablecolumns{6}
  \tablewidth{0pc}
  \tablehead{\colhead{GRB Name} & \colhead{UT Date\tablenotemark{a}} &
             \colhead{Time Since Burst\tablenotemark{b}} & \colhead{Filter} &
             \colhead{Exposure Time} & \colhead{Observed Magnitude} \\
             & & \colhead{(s)} & & \colhead{(s)} & 
            }
  \startdata
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,050412 & 2005 Apr 12.2431 & 391.0 & \Rc & 60.0 & $> 20.8$ \\
  $\cdots$ & 2005 Apr 12.2468 & 684.7 & \Rc & 180.0 & $> 21.4$ \\
  $\cdots$ & 2005 Apr 12.2512 & 1063.7 & \iG & 180.0 & $> 21.0$ \\
  $\cdots$ & 2005 Apr 12.2580 & 1646.0 & \zG & 180.0 & $> 20.2$ \\
  $\cdots$ & 2005 Apr 12.2720 & 2858.8 & \Rc & 960.0 & $> 22.5$ \\
  $\cdots$ & 2005 Apr 12.2831 & 2817.0 & \iG & 960.0 & $> 22.0$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,050416A\tablenotemark{c} & 2005 Apr 16.4641 & 216.0 & \Ic & 120.0 &
     $18.82 \pm 0.11$ \\
  $\cdots$ & 2005 Apr 16.4659 & 371.5 & \Ic & 120.0 & $18.86 \pm 0.11$ \\
  $\cdots$ & 2005 Apr 16.4677 & 527.0 & \Ic & 120.0 & $19.16 \pm 0.13$ \\
  $\cdots$ & 2005 Apr 16.4696 & 691.2 & \Ic & 120.0 & $19.35 \pm 0.23$ \\
  $\cdots$ & 2005 Apr 16.4714 & 846.7 & \Ic & 120.0 & $19.01 \pm 0.12$ \\
  $\cdots$ & 2005 Apr 16.4731 & 1002.2 & \Ic & 120.0 & $19.53 \pm 0.18$ \\
  $\cdots$ & 2005 Apr 16.4772 & 1347.8 & \zG & 360.0 & $19.16 \pm 0.27$ \\
  $\cdots$ & 2005 Apr 16.4833 & 1874.9 & \Ic & 60.0 & $19.09 \pm 0.20$ \\
  $\cdots$ & 2005 Apr 16.4880 & 2281.0 & \Ic & 60.0 & $19.34 \pm 0.23$ \\
  $\cdots$ & 2005 Apr 17.3895 & $8.017 \times 10^{4}$ & \Rc & 4320.0 & 
     $22.62 \pm 0.30$ \\
  $\cdots$ & 2005 Apr 17.4006 & $8.113 \times 10^{4}$ & \zG & 2880.0 & 
     $> 20.4$ \\
  $\cdots$ & 2005 Apr 17.4087 & $8.179 \times 10^{4}$ & \iG & 4200.0 & 
     $22.05 \pm 0.30$ \\
  $\cdots$ & 2005 Apr 18.2884 & $1.578 \times 10^{5}$ & \Rc & 8280.0 & 
     $> 23.6$ \\
  $\cdots$ & 2005 Apr 18.4031 & $1.677 \times 10^{5}$ & \iG & 8280.0 & 
     $> 22.8$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,050607 & 2005 Jun 7.3951 & 1081.0 & \Rc & 60.0 & $> 19.1$ \\
  $\cdots$ & 2005 Jun 7.3997 & 1545.0 & \Rc & 180.0 & $> 19.1$ \\
  $\cdots$ & 2005 Jun 7.4017 & 1713.2 & \iG & 180.0 & $> 18.7$ \\
  $\cdots$ & 2005 Jun 7.4029 & 1816.4 & \zG & 180.0 & $> 18.6$ \\
  $\cdots$ & 2005 Jun 7.4194 & 3334.9 & \zG & 360.0 & $> 18.6$ \\
  $\cdots$ & 2005 Jun 7.4302 & 5649.1 & \Rc & 1560.0 & $> 19.2$ \\
  $\cdots$ & 2005 Jun 7.4340 & 5851.5 & \iG & 1440.0 & $> 18.7$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,050713A & 2005 Jul 13.1960 & 821.7 & \Rc & 60.0 & $19.62 \pm 0.22$ \\
  $\cdots$ & 2005 Jul 13.2010 & 1254.1 & \Rc & 60.0 & $19.92 \pm 0.26$ \\
  $\cdots$ & 2005 Jul 13.2013 & 1341.0 & \iG & 180.0 & $19.38 \pm 0.33$ \\
  $\cdots$ & 2005 Jul 13.2040 & 1514.6 & \Rc & 60.0 & $19.92 \pm 0.26$ \\
  $\cdots$ & 2005 Jul 13.2071 & 1812.3 & \Rc & 120.0 & $19.84 \pm 0.22$ \\
  $\cdots$ & 2005 Jul 13.2139 & 2401.1 & \Rc & 120.0 & $20.19 \pm 0.28$ \\
  $\cdots$ & 2005 Jul 13.2143 & 2552.1 & \iG & 360.0 & $19.48 \pm 0.33$ \\
  $\cdots$ & 2005 Jul 13.2209 & 2999.8 & \Rc & 120.0 & $19.97 \pm 0.24$ \\
  $\cdots$ & 2005 Jul 13.2336 & 4224.4 & \iG & 360.0 & $20.22 \pm 0.40$ \\
  $\cdots$ & 2005 Jul 13.3431 & $1.386 \times 10^{4}$ & \iG & 720.0 & 
     $> 20.1$ \\
  $\cdots$ & 2005 Jul 13.3433 & $1.400 \times 10^{4}$ & \Rc & 960.0 & 
     $> 19.6$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,050820A\tablenotemark{d} & 2005 Aug 20.2766 & 236.0 & \Rc & 60.0 &
     $15.39 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.2777 & 328.0 & \iG & 60.0 & $14.91 \pm 0.02$ \\
  $\cdots$ & 2005 Aug 20.2787 & 417.0 & \zG & 60.0 & $13.93 \pm 0.11$ \\
  $\cdots$ & 2005 Aug 20.2802 & 518.0 & \Rc & 60.0 & $14.65 \pm 0.02$ \\
  $\cdots$ & 2005 Aug 20.2811 & 626.0 & \iG & 60.0 & $14.42 \pm 0.01$ \\
  $\cdots$ & 2005 Aug 20.2821 & 712.0 & \zG & 60.0 & $14.27 \pm 0.14$ \\
  $\cdots$ & 2005 Aug 20.2833 & 812.0 & \Rc & 60.0 & $15.06 \pm 0.03$ \\
  $\cdots$ & 2005 Aug 20.2844 & 913.0 & \iG & 60.0 & $14.78 \pm 0.01$ \\
  $\cdots$ & 2005 Aug 20.2856 & 1017.0 & \zG & 60.0 & $14.62 \pm 0.21$ \\
  $\cdots$ & 2005 Aug 20.2868 & 1146.0 & \Rc & 120.0 & $15.42 \pm 0.02$ \\
  $\cdots$ & 2005 Aug 20.2886 & 1304.0 & \iG & 120.0 & $15.24 \pm 0.02$ \\
  $\cdots$ & 2005 Aug 20.2905 & 1463.0 & \zG & 120.0 & $15.02 \pm 0.13$ \\
  $\cdots$ & 2005 Aug 20.2923 & 1620.0 & \gG & 120.0 & $16.27 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.2941 & 1781.0 & \Rc & 120.0 & $16.05 \pm 0.03$ \\
  $\cdots$ & 2005 Aug 20.2960 & 1942.0 & \iG & 120.0 & $15.74 \pm 0.02$ \\
  $\cdots$ & 2005 Aug 20.2979 & 2103.0 & \zG & 120.0 & $15.49 \pm 0.14$ \\
  $\cdots$ & 2005 Aug 20.2997 & 2262.0 & \gG & 120.0 & $16.62 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.3016 & 2426.0 & \Rc & 120.0 & $16.39 \pm 0.02$ \\
  $\cdots$ & 2005 Aug 20.3035 & 2590.0 & \iG & 120.0 & $16.07 \pm 0.02$ \\
  $\cdots$ & 2005 Aug 20.3054 & 2752.0 & \zG & 120.0 & $15.96 \pm 0.20$ \\
  $\cdots$ & 2005 Aug 20.3072 & 2911.0 & \gG & 120.0 & $16.92 \pm 0.05$ \\
  $\cdots$ & 2005 Aug 20.3130 & 3440.0 & \Rc & 360.0 & $16.77 \pm 0.02$ \\
  $\cdots$ & 2005 Aug 20.3175 & 3918.0 & \iG & 360.0 & $16.54 \pm 0.03$ \\
  $\cdots$ & 2005 Aug 20.3346 & 5394.0 & \gG & 360.0 & $17.59 \pm 0.05$ \\
  $\cdots$ & 2005 Aug 20.3413 & 5885.0 & \Rc & 360.0 & $17.32 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.3460 & 6382.0 & \iG & 360.0 & $17.02 \pm 0.05$ \\
  $\cdots$ & 2005 Aug 20.3519 & 6889.0 & \gG & 360.0 & $17.87 \pm 0.06$ \\
  $\cdots$ & 2005 Aug 20.3587 & 7392.0 & \Rc & 360.0 & $17.48 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.3635 & 7893.0 & \iG & 360.0 & $17.22 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.3693 & 8397.0 & \gG & 360.0 & $18.11 \pm 0.06$ \\
  $\cdots$ & 2005 Aug 20.3763 & 8906.0 & \Rc & 360.0 & $17.69 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.3811 & 9414.0 & \iG & 360.0 & $17.23 \pm 0.05$ \\
  $\cdots$ & 2005 Aug 20.3940 & $1.044 \times 10^{4}$ & \Rc & 360.0 &
     $17.85 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.3940 & $1.070 \times 10^{4}$ & \gG & 720.0 &
     $18.29 \pm 0.06$ \\
  $\cdots$ & 2005 Aug 20.3989 & $1.095 \times 10^{4}$ & \iG & 360.0 &
     $17.34 \pm 0.03$ \\
  $\cdots$ & 2005 Aug 20.4161 & $1.235 \times 10^{4}$ & \Rc & 360.0 &
     $17.78 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.4292 & $1.357 \times 10^{4}$ & \iG & 360.0 &
     $17.48 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.4427 & $1.465 \times 10^{4}$ & \Rc & 360.0 &
     $17.97 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.4357 & $1.491 \times 10^{4}$ & \gG & 720.0 &
     $18.36 \pm 0.06$ \\
  $\cdots$ & 2005 Aug 20.4479 & $1.518 \times 10^{4}$ & \iG & 360.0 &
     $17.68 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.4614 & $1.626 \times 10^{4}$ & \Rc & 360.0 &
     $18.01 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.4666 & $1.680 \times 10^{4}$ & \iG & 360.0 &
     $17.71 \pm 0.05$ \\
  $\cdots$ & 2005 Aug 20.4804 & $1.790 \times 10^{4}$ & \Rc & 360.0 & 
     $18.03 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.4816 & $1.828 \times 10^{4}$ & \gG & 720.0 &
     $18.59 \pm 0.09$ \\
  $\cdots$ & 2005 Aug 20.4857 & $1.845 \times 10^{4}$ & \iG & 360.0 &
     $17.72 \pm 0.04$ \\
  $\cdots$ & 2005 Aug 20.5007 & $1.966 \times 10^{4}$ & \Rc & 360.0 & 
     $18.16 \pm 0.05$ \\
  $\cdots$ & 2005 Aug 22.2243 & $1.753 \times 10^{5}$ & \Rc & 6840.0 & 
     $20.51 \pm 0.11$ \\
  $\cdots$ & 2005 Aug 22.2299 & $1.758 \times 10^{5}$ & \iG & 6840.0 & 
     $19.97 \pm 0.12$ \\
  $\cdots$ & 2005 Aug 23.2404 & $2.647 \times 10^{5}$ & \Rc & 8400.0 & 
     $20.89 \pm 0.10$ \\
  $\cdots$ & 2005 Aug 23.2616 & $2.657 \times 10^{5}$ & \iG & 7560.0 &
     $20.48 \pm 0.12$ \\
  $\cdots$ & 2005 Aug 24.2684 & $3.535 \times 10^{5}$ & \Rc & 8400.0 & 
     $21.22 \pm 0.11$ \\
  $\cdots$ & 2005 Aug 24.2860 & $3.550 \times 10^{5}$ & \iG & 8400.0 &
     $20.59 \pm 0.11$ \\
  $\cdots$ & 2005 Aug 25.3647 & $4.427 \times 10^{5}$ & \Rc & 2880.0 & 
     $21.34 \pm 0.13$ \\
  $\cdots$ & 2005 Aug 25.4199 & $4.470 \times 10^{5}$ & \iG & 2400.0 &
     $21.02 \pm 0.15$ \\
  $\cdots$ & 2005 Aug 26.3113 & $5.252 \times 10^{5}$ & \Rc & 3600.0 & 
     $21.64 \pm 0.12$ \\
  $\cdots$ & 2005 Aug 26.3385 & $5.288 \times 10^{5}$ & \iG & 4800.0 &
     $21.17 \pm 0.14$ \\
  $\cdots$ & 2005 Aug 27.3056 & $6.120 \times 10^{5}$ & \iG & 4440.0 &
     $21.30 \pm 0.13$ \\
  $\cdots$ & 2005 Aug 27.3036 & $6.121 \times 10^{5}$ & \Rc & 4800.0 &
     $21.80 \pm 0.12$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,050908 & 2005 Sep 8.2408 & 279.9 & \Rc & 60.0 & $18.46 \pm 0.13$ \\
  $\cdots$ & 2005 Sep 8.2418 & 372.3 & \iG & 60.0 & $18.10 \pm 0.16$ \\
  $\cdots$ & 2005 Sep 8.2440 & 562.4 & \Rc & 60.0 & $18.99 \pm 0.19$ \\
  $\cdots$ & 2005 Sep 8.2451 & 656.2 & \iG & 60.0 & $18.02 \pm 0.14$ \\
  $\cdots$ & 2005 Sep 8.2474 & 850.7 & \Rc & 60.0 & $19.28 \pm 0.22$ \\
  $\cdots$ & 2005 Sep 8.2477 & 941.6 & \zG & 180.0 & $> 18.2$ \\
  $\cdots$ & 2005 Sep 8.2486 & 955.4 & \iG & 60.0 & $18.66 \pm 0.21$ \\
  $\cdots$ & 2005 Sep 8.2573 & 1742.4 & \Rc & 120.0 & $19.37 \pm 0.15$ \\
  $\cdots$ & 2005 Sep 8.2650 & 2400.9 & \Rc & 120.0 & $19.54 \pm 0.16$ \\
  $\cdots$ & 2005 Sep 8.2655 & 2569.5 & \iG & 360.0 & $19.20 \pm 0.14$ \\
  $\cdots$ & 2005 Sep 8.2674 & 2735.3 & \zG & 360.0 & $> 19.3$ \\
  $\cdots$ & 2005 Sep 8.2727 & 3069.9 & \Rc & 120.0 & $19.80 \pm 0.19$ \\
  $\cdots$ & 2005 Sep 8.3206 & 7598.4 & \Rc & 900.0 & $20.68 \pm 0.14$ \\
  $\cdots$ & 2005 Sep 8.2655 & 2569.5 & \iG & 360.0 & $19.20 \pm 0.14$ \\
  $\cdots$ & 2005 Sep 8.4723 & $2.071 \times 10^{4}$ & \Rc & 900.0 & 
     $21.62 \pm 0.24$ \\
  $\cdots$ & 2005 Sep 8.4905 & $2.237 \times 10^{4}$ & \iG & 1080.0 & 
     $20.70 \pm 0.16$ \\
  $\cdots$ & 2005 Sep 8.5011 & $2.319 \times 10^{4}$ & \Rc & 900.0 & 
     $21.66 \pm 0.28$ \\
  $\cdots$ & 2005 Sep 9.2955 & $9.273 \times 10^{4}$ & \iG & 2700.0 &
     $> 21.3$ \\
  $\cdots$ & 2005 Sep 9.2968 & $9.320 \times 10^{4}$ & \Rc & 3420.0 & 
     $> 22.3$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,050915A & 2005 Sep 15.4767 & 257.0 & \Rc & 60.0 & $> 20.3$ \\
  $\cdots$ & 2005 Sep 15.4780 & 365.5 & \iG & 60.0 & $> 19.6$ \\
  $\cdots$ & 2005 Sep 15.4792 & 472.5 & \zG & 60.0 & $> 19.1$ \\
  $\cdots$ & 2005 Sep 15.4799 & 501.1 & \Rc & 180.0 & $> 20.7$ \\
  $\cdots$ & 2005 Sep 15.4812 & 611.5 & \iG & 180.0 & $> 20.5$ \\
  $\cdots$ & 2005 Sep 15.4824 & 721.5 & \zG & 180.0 & $> 19.6$ \\
  $\cdots$ & 2005 Sep 15.4963 & 1916.6 & \Rc & 360.0 & $> 21.1$ \\
  $\cdots$ & 2005 Sep 15.4986 & 2117.9 & \iG & 360.0 & $> 21.0$ \\
  $\cdots$ & 2005 Sep 15.5009 & 2319.4 & \zG & 360.0 & $> 20.0$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,060110 & 2006 Jan 10.3493 & 1334.5 & \Rc & 60.0 & $17.45 \pm 0.22$ \\
  $\cdots$ & 2006 Jan 10.3590 & 2170.0 & \ip & 60.0 & $17.45 \pm 0.20$ \\
  $\cdots$ & 2006 Jan 10.3608 & 2312.8 & \ip & 30.0 & $17.46 \pm 0.21$ \\
  $\cdots$ & 2006 Jan 10.3621 & 2424.5 & \ip & 30.0 & $17.77 \pm 0.23$ \\
  $\cdots$ & 2006 Jan 10.3634 & 2538.9 & \ip & 30.0 & $17.83 \pm 0.26$ \\
  $\cdots$ & 2006 Jan 10.3647 & 2648.0 & \ip & 30.0 & $17.85 \pm 0.25$ \\
  $\cdots$ & 2006 Jan 10.3660 & 2758.8 & \ip & 30.0 & $17.55 \pm 0.22$ \\
  $\cdots$ & 2006 Jan 10.3674 & 2883.9 & \ip & 30.0 & $17.80 \pm 0.23$ \\
  $\cdots$ & 2006 Jan 10.3687 & 2992.6 & \ip & 30.0 & $17.87 \pm 0.24$ \\
  $\cdots$ & 2006 Jan 10.3700 & 3104.7 & \ip & 30.0 & $17.95 \pm 0.28$ \\
  $\cdots$ & 2006 Jan 10.4083 & 6476.3 & \ip & 150.0 & $18.60 \pm 0.24$ \\
  $\cdots$ & 2006 Jan 10.4322 & 8536.1 & \ip & 150.0 & $> 18.8$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,060210 & 2006 Feb 10.2105 & 289.2 & \Rc & 60.0 & $18.22 \pm 0.26$ \\
  $\cdots$ & 2006 Feb 10.2115 & 377.9 & \Rc & 60.0 & $18.60 \pm 0.29$ \\
  $\cdots$ & 2006 Feb 10.2138 & 569.4 & \zp & 60.0 & $16.05 \pm 0.41$ \\
  $\cdots$ & 2006 Feb 10.2148 & 662.6 & \Rc & 60.0 & $18.29 \pm 0.29$ \\
  $\cdots$ & 2006 Feb 10.2160 & 760.8 & \ip & 60.0 & $17.34 \pm 0.22$ \\
  $\cdots$ & 2006 Feb 10.2171 & 855.5 & \zp & 60.0 & $16.64 \pm 0.36$ \\
  $\cdots$ & 2006 Feb 10.2182 & 950.3 & \Rc & 60.0 & $18.35 \pm 0.27$ \\
  $\cdots$ & 2006 Feb 10.2193 & 1044.9 & \ip & 60.0 & $17.78 \pm 0.21$ \\
  $\cdots$ & 2006 Feb 10.2204 & 1140.6 & \zp & 60.0 & $16.98 \pm 0.38$ \\
  $\cdots$ & 2006 Feb 10.2215 & 1265.7 & \Rc & 120.0 & $19.25 \pm 0.30$ \\
  $\cdots$ & 2006 Feb 10.2233 & 1425.1 & \ip & 120.0 & $18.18 \pm 0.21$ \\
  $\cdots$ & 2006 Feb 10.2330 & 2262.9 & \Rc & 120.0 & $19.77 \pm 0.26$ \\
  $\cdots$ & 2006 Feb 10.2349 & 2422.1 & \ip & 120.0 & $19.12 \pm 0.23$ \\
  $\cdots$ & 2006 Feb 10.2386 & 2743.7 & \Rc & 120.0 & $20.28 \pm 0.31$ \\
  $\cdots$ & 2006 Feb 10.2404 & 2904.8 & \ip & 120.0 & $19.06 \pm 0.20$ \\
  $\cdots$ & 2006 Feb 10.2430 & 3304.4 & \gG & 480.0 & $> 20.2$ \\
  $\cdots$ & 2006 Feb 10.2460 & 3387.9 & \ip & 120.0 & $19.25 \pm 0.20$ \\
  $\cdots$ & 2006 Feb 10.2484 & 3710.8 & \Rc & 360.0 & $20.17 \pm 0.26$ \\
  $\cdots$ & 2006 Feb 10.2516 & 3870.3 & \ip & 120.0 & $19.51 \pm 0.21$ \\
  $\cdots$ & 2006 Feb 10.2570 & 4501.8 & \Rc & 450.0 & $20.86 \pm 0.32$ \\
  $\cdots$ & 2006 Feb 10.2636 & 5068.1 & \ip & 450.0 & $20.08 \pm 0.21$ \\
  $\cdots$ & 2006 Feb 10.2833 & 6768.5 & \ip & 450.0 & $20.17 \pm 0.23$ \\
  $\cdots$ & 2006 Feb 10.2845 & 7105.1 & \Rc & 900.0 & $20.91 \pm 0.30$ \\
  $\cdots$ & 2006 Feb 10.2853 & 7391.3 & \gG & 1350.0 & $> 20.3$ \\
  $\cdots$ & 2006 Feb 10.3124 & 9511.9 & \ip & 900.0 & $20.41 \pm 0.23$ \\
  $\cdots$ & 2006 Feb 10.3271 & $1.078 \times 10^{4}$ & \Rc & 900.0 &
     $> 20.8$ \\
  $\cdots$ & 2006 Feb 11.1063 & $7.915 \times 10^{4}$ & \ip & 3000.0 & 
     $> 22.5$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,060502A & 2006 May 2.1536 & 2287.2 & \Rc & 60.0 & $19.93 \pm 0.19$ \\
  $\cdots$ & 2006 May 2.1549 & 2397.3 & \ip & 60.0 & $19.67 \pm 0.27$ \\
  $\cdots$ & 2006 May 2.1561 & 2508.5 & \zp & 60.0 & $20.43 \pm 0.71$ \\
  $\cdots$ & 2006 May 2.1574 & 2619.4 & \Rc & 60.0 & $20.18 \pm 0.21$ \\
  $\cdots$ & 2006 May 2.1586 & 2725.1 & \ip & 60.0 & $19.93 \pm 0.29$ \\
  $\cdots$ & 2006 May 2.1600 & 2838.6 & \zp & 60.0 & $19.20 \pm 0.71$ \\
  $\cdots$ & 2006 May 2.1613 & 2982.9 & \Rc & 120.0 & $19.88 \pm 0.15$ \\
  $\cdots$ & 2006 May 2.1634 & 3168.1 & \ip & 120.0 & $20.03 \pm 0.29$ \\
  $\cdots$ & 2006 May 2.1677 & 3537.1 & \gG & 120.0 & $21.18 \pm 0.35$ \\
  $\cdots$ & 2006 May 2.1697 & 3708.2 & \Rc & 120.0 & $20.45 \pm 0.18$ \\
  $\cdots$ & 2006 May 2.1718 & 3892.4 & \ip & 120.0 & $20.23 \pm 0.30$ \\
  $\cdots$ & 2006 May 2.1727 & 4088.6 & \zp & 360.0 & $19.68 \pm 0.49$ \\
  $\cdots$ & 2006 May 2.1762 & 4267.4 & \gG & 120.0 & $21.35 \pm 0.37$ \\
  $\cdots$ & 2006 May 2.1783 & 4454.1 & \Rc & 120.0 & $20.23 \pm 0.17$ \\
  $\cdots$ & 2006 May 2.1805 & 4642.6 & \ip & 120.0 & $20.07 \pm 0.28$ \\
  $\cdots$ & 2006 May 2.1848 & 5016.4 & \gG & 120.0 & $21.48 \pm 0.38$ \\
  $\cdots$ & 2006 May 2.1980 & 6318.2 & \Rc & 450.0 & $20.41 \pm 0.14$ \\
  $\cdots$ & 2006 May 2.2054 & 6956.9 & \gG & 450.0 & $21.62 \pm 0.33$ \\
  $\cdots$ & 2006 May 2.2127 & 7591.7 & \ip & 450.0 & $20.51 \pm 0.29$ \\
  $\cdots$ & 2006 May 2.2201 & 8228.6 & \Rc & 450.0 & $20.50 \pm 0.14$ \\
  $\cdots$ & 2006 May 2.2275 & 8870.9 & \gG & 450.0 & $21.81 \pm 0.34$ \\
  $\cdots$ & 2006 May 2.2349 & 9509.8 & \ip & 450.0 & $20.44 \pm 0.28$ \\
  $\cdots$ & 2006 May 2.2423 & $1.015 \times 10^{4}$ & \Rc & 450.0 & 
     $20.74 \pm 0.15$ \\
  $\cdots$ & 2006 May 2.2498 & $1.079 \times 10^{4}$ & \gG & 450.0 & 
     $21.84 \pm 0.34$ \\
  $\cdots$ & 2006 May 2.2700 & $1.254 \times 10^{4}$ & \ip & 450.0 & 
     $20.81 \pm 0.29$ \\
  $\cdots$ & 2006 May 3.2888 & $1.019 \times 10^{5}$ & \ip & 3150.0 & 
     $22.01 \pm 0.33$ \\
  $\cdots$ & 2006 May 3.2951 & $1.025 \times 10^{5}$ & \Rc & 3150.0 & 
     $22.08 \pm 0.22$ \\
  $\cdots$ & 2006 May 3.3023 & $1.047 \times 10^{5}$ & \gG & 3150.0 &
     $> 22.9$ \\
  $\cdots$ & 2006 May 4.1513 & $1.756 \times 10^{5}$ & \ip & 1500.0 &
     $> 21.4$ \\
  $\cdots$ & 2006 May 4.1709 & $1.773 \times 10^{5}$ & \Rc & 1500.0 &
     $> 21.4$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,060510B & 2006 May 10.3671 & 1610.7 & \Rc & 60.0 & $> 19.5$ \\
  $\cdots$ & 2006 May 10.3681 & 1698.0 & \ip & 60.0 & $> 20.3$ \\
  $\cdots$ & 2006 May 10.3692 & 1793.5 & \zp & 60.0 & $19.51 \pm 0.71$ \\
  $\cdots$ & 2006 May 10.3696 & 1892.3 & \Rc & 180.0 & $> 20.2$ \\
  $\cdots$ & 2006 May 10.3707 & 1983.5 & \ip & 180.0 & $> 20.3$ \\
  $\cdots$ & 2006 May 10.3718 & 2079.7 & \zp & 180.0 & $19.68 \pm 0.71$ \\
  $\cdots$ & 2006 May 10.3828 & 3117.1 & \Rc & 360.0 & $> 20.7$ \\
  $\cdots$ & 2006 May 10.3846 & 3272.3 & \ip & 360.0 & $21.19 \pm 0.45$ \\
  $\cdots$ & 2006 May 10.3864 & 3430.1 & \zp & 360.0 & $19.77 \pm 0.68$ \\
  $\cdots$ & 2006 May 10.3882 & 3585.8 & \gG & 360.0 & $> 21.4$ \\
  $\cdots$ & 2006 May 10.4240 & 7397.9 & \Rc & 1800.0 & $21.68 \pm 0.25$ \\
  $\cdots$ & 2006 May 10.4393 & 8628.7 & \ip & 1620.0 & $21.31 \pm 0.39$ \\
  $\cdots$ & 2006 May 10.4494 & 9597.6 & \zp & 1800.0 & $20.48 \pm 0.67$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,060805A & 2006 Aug 5.2020 & 214.4 & \Rc & 60.0 & $> 20.0$ \\
  $\cdots$ & 2006 Aug 5.2030 & 304.7 & \ip & 60.0 & $> 20.4$ \\
  $\cdots$ & 2006 Aug 5.2042 & 402.6 & \zp & 60.0 & $> 19.7$ \\
  $\cdots$ & 2006 Aug 5.2044 & 447.2 & \ip & 180.0 & $> 20.7$ \\
  $\cdots$ & 2006 Aug 5.2055 & 543.7 & \zp & 120.0 & $> 20.0$ \\
  $\cdots$ & 2006 Aug 5.2127 & 1196.7 & \Rc & 180.0 & $> 20.3$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,060906 & 2006 Sep 6.3634 & 661.0 & \Rc & 60.0 & $19.18 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 6.3646 & 765.2 & \ip & 60.0 & $18.73 \pm 0.23$ \\
  $\cdots$ & 2006 Sep 6.3659 & 874.0 & \zp & 60.0 & $18.85 \pm 0.37$ \\
  $\cdots$ & 2006 Sep 6.3671 & 983.4 & \Rc & 60.0 & $18.98 \pm 0.14$ \\
  $\cdots$ & 2006 Sep 6.3683 & 1087.8 & \ip & 60.0 & $18.87 \pm 0.25$ \\
  $\cdots$ & 2006 Sep 6.3700 & 1229.3 & \zp & 60.0 & $18.79 \pm 0.35$ \\
  $\cdots$ & 2006 Sep 6.3712 & 1336.5 & \Rc & 60.0 & $19.14 \pm 0.15$ \\
  $\cdots$ & 2006 Sep 6.3725 & 1445.3 & \ip & 60.0 & $18.95 \pm 0.19$ \\
  $\cdots$ & 2006 Sep 6.3737 & 1555.5 & \zp & 60.0 & $18.78 \pm 0.50$ \\
  $\cdots$ & 2006 Sep 6.3750 & 1696.3 & \Rc & 120.0 & $19.35 \pm 0.14$ \\
  $\cdots$ & 2006 Sep 6.3772 & 1885.3 & \ip & 120.0 & $19.21 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.3794 & 2073.7 & \zp & 120.0 & $19.23 \pm 0.37$ \\
  $\cdots$ & 2006 Sep 6.3815 & 2254.0 & \gG & 120.0 & $20.82 \pm 0.22$ \\
  $\cdots$ & 2006 Sep 6.3836 & 2437.7 & \Rc & 120.0 & $19.61 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.3857 & 2622.5 & \ip & 120.0 & $19.46 \pm 0.23$ \\
  $\cdots$ & 2006 Sep 6.3879 & 2810.6 & \zp & 120.0 & $19.65 \pm 0.38$ \\
  $\cdots$ & 2006 Sep 6.3901 & 2995.9 & \gG & 120.0 & $20.69 \pm 0.26$ \\
  $\cdots$ & 2006 Sep 6.3922 & 3183.7 & \Rc & 120.0 & $19.95 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 6.3945 & 3378.2 & \ip & 120.0 & $19.71 \pm 0.32$ \\
  $\cdots$ & 2006 Sep 6.3967 & 3565.0 & \zp & 120.0 & $20.02 \pm 0.39$ \\
  $\cdots$ & 2006 Sep 6.3989 & 3755.2 & \gG & 120.0 & $20.98 \pm 0.22$ \\
  $\cdots$ & 2006 Sep 6.4038 & 4180.1 & \Rc & 120.0 & $20.08 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 6.4058 & 4356.9 & \Rc & 120.0 & $20.23 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.4079 & 4532.3 & \Rc & 120.0 & $20.25 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.4100 & 4715.6 & \ip & 120.0 & $20.08 \pm 0.19$ \\
  $\cdots$ & 2006 Sep 6.4120 & 4892.5 & \ip & 120.0 & $20.22 \pm 0.20$ \\
  $\cdots$ & 2006 Sep 6.4141 & 5075.6 & \ip & 120.0 & $20.17 \pm 0.20$ \\
  $\cdots$ & 2006 Sep 6.4163 & 5264.5 & \zp & 120.0 & $20.07 \pm 0.38$ \\
  $\cdots$ & 2006 Sep 6.4183 & 5438.2 & \zp & 120.0 & $19.86 \pm 0.35$ \\
  $\cdots$ & 2006 Sep 6.4204 & 5618.4 & \zp & 120.0 & $19.93 \pm 0.36$ \\
  $\cdots$ & 2006 Sep 6.4227 & 5811.0 & \gG & 120.0 & $21.52 \pm 0.28$ \\
  $\cdots$ & 2006 Sep 6.4247 & 5987.7 & \gG & 120.0 & $21.09 \pm 0.22$ \\
  $\cdots$ & 2006 Sep 6.4268 & 6168.8 & \gG & 120.0 & $21.33 \pm 0.26$ \\
  $\cdots$ & 2006 Sep 6.4290 & 6357.6 & \Rc & 120.0 & $19.97 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 6.4310 & 6533.3 & \Rc & 120.0 & $19.68 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.4331 & 6718.0 & \Rc & 120.0 & $19.75 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 6.4353 & 6901.6 & \ip & 120.0 & $19.63 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.4374 & 7082.7 & \ip & 120.0 & $19.48 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.4395 & 7264.9 & \ip & 120.0 & $19.48 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.4417 & 7453.1 & \zp & 120.0 & $19.29 \pm 0.37$ \\
  $\cdots$ & 2006 Sep 6.4437 & 7632.2 & \zp & 120.0 & $19.05 \pm 0.35$ \\
  $\cdots$ & 2006 Sep 6.4459 & 7816.4 & \zp & 120.0 & $19.16 \pm 0.36$ \\
  $\cdots$ & 2006 Sep 6.4480 & 8001.3 & \gG & 120.0 & $20.54 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.4501 & 8184.1 & \gG & 120.0 & $20.34 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.4522 & 8365.9 & \gG & 120.0 & $20.37 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.4544 & 8553.6 & \Rc & 120.0 & $19.31 \pm 0.15$ \\
  $\cdots$ & 2006 Sep 6.4565 & 8731.5 & \Rc & 120.0 & $19.27 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 6.4585 & 8909.2 & \Rc & 120.0 & $19.31 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 6.4606 & 9091.7 & \ip & 120.0 & $19.10 \pm 0.19$ \\
  $\cdots$ & 2006 Sep 6.4628 & 9276.9 & \ip & 120.0 & $19.07 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.4649 & 9457.7 & \ip & 120.0 & $19.09 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.4670 & 9644.3 & \zp & 120.0 & $18.95 \pm 0.36$ \\
  $\cdots$ & 2006 Sep 6.4692 & 9829.0 & \zp & 120.0 & $18.91 \pm 0.35$ \\
  $\cdots$ & 2006 Sep 6.4713 & $1.001 \times 10^{4}$ & \zp & 120.0 & 
     $18.85 \pm 0.35$ \\
  $\cdots$ & 2006 Sep 6.4734 & $1.020 \times 10^{4}$ & \gG & 120.0 & 
     $20.36 \pm 0.19$ \\
  $\cdots$ & 2006 Sep 6.4755 & $1.038 \times 10^{4}$ & \gG & 120.0 & 
     $20.36 \pm 0.19$ \\
  $\cdots$ & 2006 Sep 6.4776 & $1.056 \times 10^{4}$ & \gG & 120.0 & 
     $20.32 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.4798 & $1.075 \times 10^{4}$ & \Rc & 120.0 & 
     $19.21 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.4819 & $1.093 \times 10^{4}$ & \Rc & 120.0 & 
     $19.22 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.4841 & $1.112 \times 10^{4}$ & \Rc & 120.0 & 
     $19.24 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.4862 & $1.130 \times 10^{4}$ & \ip & 120.0 & 
     $19.11 \pm 0.18$ \\
  $\cdots$ & 2006 Sep 6.4915 & $1.176 \times 10^{4}$ & \ip & 120.0 & 
     $19.10 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.4935 & $1.194 \times 10^{4}$ & \ip & 120.0 & 
     $19.14 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.4957 & $1.213 \times 10^{4}$ & \zp & 120.0 & 
     $18.89 \pm 0.34$ \\
  $\cdots$ & 2006 Sep 6.4979 & $1.231 \times 10^{4}$ & \zp & 120.0 & 
     $18.98 \pm 0.35$ \\
  $\cdots$ & 2006 Sep 6.5000 & $1.249 \times 10^{4}$ & \zp & 120.0 & 
     $18.96 \pm 0.35$ \\
  $\cdots$ & 2006 Sep 6.5022 & $1.268 \times 10^{4}$ & \gG & 120.0 & 
     $20.46 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.5043 & $1.286 \times 10^{4}$ & \gG & 120.0 & 
     $20.41 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.5065 & $1.305 \times 10^{4}$ & \gG & 120.0 & 
     $20.48 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 6.5087 & $1.324 \times 10^{4}$ & \Rc & 120.0 & 
     $19.31 \pm 0.14$ \\
  $\cdots$ & 2006 Sep 6.5107 & $1.342 \times 10^{4}$ & \Rc & 120.0 & 
     $19.32 \pm 0.14$ \\
  $\cdots$ & 2006 Sep 6.5129 & $1.361 \times 10^{4}$ & \Rc & 120.0 & 
     $19.36 \pm 0.14$ \\
  $\cdots$ & 2006 Sep 6.5151 & $1.379 \times 10^{4}$ & \ip & 120.0 & 
     $19.21 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.5172 & $1.398 \times 10^{4}$ & \ip & 120.0 & 
     $19.25 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.5192 & $1.415 \times 10^{4}$ & \ip & 120.0 & 
     $19.20 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 6.5215 & $1.435 \times 10^{4}$ & \zp & 120.0 & 
     $19.01 \pm 0.35$ \\
  $\cdots$ & 2006 Sep 7.4582 & $9.618 \times 10^{4}$ & \Rc & 1920.0 &
     $> 21.9$ \\
  $\cdots$ & 2006 Sep 7.4570 & $9.620 \times 10^{4}$ & \ip & 2160.0 &
     $> 22.0$ \\
  $\cdots$ & 2006 Sep 7.4589 & $9.625 \times 10^{4}$ & \gG & 1920.0 &
     $> 22.3$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,060908 & 2006 Sep 8.3824 & 825.2 & \Rc & 60.0 & $17.51 \pm 0.05$ \\
  $\cdots$ & 2006 Sep 8.3854 & 1082.6 & \ip & 60.0 & $17.86 \pm 0.05$ \\
  $\cdots$ & 2006 Sep 8.3864 & 1171.6 & \Rc & 60.0 & $17.85 \pm 0.06$ \\
  $\cdots$ & 2006 Sep 8.3874 & 1261.7 & \ip & 60.0 & $17.91 \pm 0.05$ \\
  $\cdots$ & 2006 Sep 8.3885 & 1354.7 & \zp & 60.0 & $17.86 \pm 0.07$ \\
  $\cdots$ & 2006 Sep 8.3896 & 1448.0 & \Rc & 60.0 & $17.95 \pm 0.06$ \\
  $\cdots$ & 2006 Sep 8.3906 & 1537.7 & \ip & 60.0 & $18.15 \pm 0.13$ \\
  $\cdots$ & 2006 Sep 8.3917 & 1632.6 & \zp & 60.0 & $18.24 \pm 0.11$ \\
  $\cdots$ & 2006 Sep 8.3949 & 1911.5 & \Rc & 60.0 & $18.20 \pm 0.05$ \\
  $\cdots$ & 2006 Sep 8.3959 & 1997.7 & \ip & 60.0 & $18.53 \pm 0.05$ \\
  $\cdots$ & 2006 Sep 8.3970 & 2088.1 & \zp & 60.0 & $18.40 \pm 0.07$ \\
  $\cdots$ & 2006 Sep 8.3980 & 2174.5 & \gG & 60.0 & $19.03 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 8.3990 & 2263.1 & \Rc & 60.0 & $18.40 \pm 0.05$ \\
  $\cdots$ & 2006 Sep 8.4001 & 2357.7 & \ip & 60.0 & $18.57 \pm 0.05$ \\
  $\cdots$ & 2006 Sep 8.4012 & 2452.5 & \zp & 60.0 & $18.43 \pm 0.07$ \\
  $\cdots$ & 2006 Sep 8.4022 & 2539.4 & \gG & 60.0 & $19.13 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 8.4033 & 2633.9 & \Rc & 60.0 & $18.72 \pm 0.07$ \\
  $\cdots$ & 2006 Sep 8.4043 & 2720.7 & \ip & 60.0 & $18.80 \pm 0.06$ \\
  $\cdots$ & 2006 Sep 8.4054 & 2816.7 & \zp & 60.0 & $18.50 \pm 0.07$ \\
  $\cdots$ & 2006 Sep 8.4064 & 2904.7 & \gG & 60.0 & $19.26 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 8.4076 & 3001.7 & \Rc & 60.0 & $18.86 \pm 0.08$ \\
  $\cdots$ & 2006 Sep 8.4086 & 3089.2 & \ip & 60.0 & $18.95 \pm 0.06$ \\
  $\cdots$ & 2006 Sep 8.4096 & 3180.7 & \zp & 60.0 & $18.95 \pm 0.11$ \\
  $\cdots$ & 2006 Sep 8.4107 & 3269.1 & \gG & 60.0 & $19.57 \pm 0.15$ \\
  $\cdots$ & 2006 Sep 8.4118 & 3367.8 & \Rc & 60.0 & $19.07 \pm 0.09$ \\
  $\cdots$ & 2006 Sep 8.4128 & 3456.3 & \ip & 60.0 & $18.88 \pm 0.06$ \\
  $\cdots$ & 2006 Sep 8.4139 & 3552.1 & \zp & 60.0 & $19.01 \pm 0.12$ \\
  $\cdots$ & 2006 Sep 8.4150 & 3640.8 & \gG & 60.0 & $19.59 \pm 0.15$ \\
  $\cdots$ & 2006 Sep 8.4160 & 3730.7 & \Rc & 60.0 & $19.10 \pm 0.09$ \\
  $\cdots$ & 2006 Sep 8.4170 & 3819.1 & \ip & 60.0 & $19.21 \pm 0.08$ \\
  $\cdots$ & 2006 Sep 8.4181 & 3912.0 & \zp & 60.0 & $18.97 \pm 0.11$ \\
  $\cdots$ & 2006 Sep 8.4191 & 4001.1 & \gG & 60.0 & $19.70 \pm 0.19$ \\
  $\cdots$ & 2006 Sep 8.4202 & 4091.5 & \Rc & 60.0 & $19.28 \pm 0.11$ \\
  $\cdots$ & 2006 Sep 8.4213 & 4187.5 & \ip & 60.0 & $19.14 \pm 0.07$ \\
  $\cdots$ & 2006 Sep 8.4224 & 4280.6 & \zp & 60.0 & $19.48 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 8.4234 & 4370.4 & \gG & 60.0 & $19.85 \pm 0.17$ \\
  $\cdots$ & 2006 Sep 8.4245 & 4491.8 & \Rc & 120.0 & $19.17 \pm 0.07$ \\
  $\cdots$ & 2006 Sep 8.4263 & 4649.4 & \ip & 120.0 & $19.38 \pm 0.10$ \\
  $\cdots$ & 2006 Sep 8.4282 & 4840.9 & \zp & 180.0 & $19.56 \pm 0.11$ \\
  $\cdots$ & 2006 Sep 8.4332 & 5249.4 & \Rc & 120.0 & $19.39 \pm 0.09$ \\
  $\cdots$ & 2006 Sep 8.4351 & 5408.0 & \ip & 120.0 & $19.70 \pm 0.09$ \\
  $\cdots$ & 2006 Sep 8.4369 & 5599.1 & \zp & 180.0 & $19.73 \pm 0.13$ \\
  $\cdots$ & 2006 Sep 8.4374 & 5822.8 & \gG & 540.0 & $20.08 \pm 0.11$ \\
  $\cdots$ & 2006 Sep 8.4421 & 6013.3 & \Rc & 120.0 & $19.65 \pm 0.11$ \\
  $\cdots$ & 2006 Sep 8.4439 & 6174.1 & \ip & 120.0 & $19.64 \pm 0.07$ \\
  $\cdots$ & 2006 Sep 8.4458 & 6367.4 & \zp & 180.0 & $19.52 \pm 0.10$ \\
  $\cdots$ & 2006 Sep 8.4510 & 6813.4 & \Rc & 180.0 & $19.99 \pm 0.13$ \\
  $\cdots$ & 2006 Sep 8.4535 & 7026.5 & \Rc & 180.0 & $19.54 \pm 0.09$ \\
  $\cdots$ & 2006 Sep 8.4560 & 7242.1 & \Rc & 180.0 & $19.72 \pm 0.09$ \\
  $\cdots$ & 2006 Sep 8.4585 & 7461.9 & \ip & 180.0 & $20.16 \pm 0.09$ \\
  $\cdots$ & 2006 Sep 8.4610 & 7676.0 & \ip & 180.0 & $20.13 \pm 0.11$ \\
  $\cdots$ & 2006 Sep 8.4634 & 7889.4 & \ip & 180.0 & $20.09 \pm 0.10$ \\
  $\cdots$ & 2006 Sep 8.4665 & 8332.8 & \zp & 540.0 & $20.49 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 8.4748 & 9052.4 & \gG & 540.0 & $20.51 \pm 0.16$ \\
  $\cdots$ & 2006 Sep 9.3843 & $8.982 \times 10^{4}$ & \ip & 4680.0 & 
    $23.16 \pm 0.30$ \\
  $\cdots$ & 2006 Sep 9.3905 & $9.036 \times 10^{4}$ & \Rc & 4680.0 & 
    $> 22.7$ \\ 
  $\cdots$ & 2006 Sep 12.3291 & $3.440 \times 10^{5}$ & \ip & 4320.0 & 
    $23.17 \pm 0.24$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,060923A & 2006 Sep 23.2205 & 348.6 & \Rc & 60.0 & $> 20.3$ \\
  $\cdots$ & 2006 Sep 23.2216 & 442.9 & \ip & 60.0 & $> 20.4$ \\ 
  $\cdots$ & 2006 Sep 23.2227 & 536.4 & \zp & 60.0 & $> 19.5$ \\
  $\cdots$ & 2006 Sep 23.2231 & 631.5 & \Rc & 180.0 & $> 20.9$ \\
  $\cdots$ & 2006 Sep 23.2242 & 725.1 & \ip & 180.0 & $> 20.9$ \\
  $\cdots$ & 2006 Sep 23.2253 & 823.5 & \zp & 180.0 & $> 19.4$ \\
  $\cdots$ & 2006 Sep 23.2431 & 2448.7 & \ip & 360.0 & $> 20.9$ \\
  $\cdots$ & 2006 Sep 23.2450 & 2611.9 & \zp & 360.0 & $> 19.7$ \\
  $\cdots$ & 2006 Sep 23.2449 & 2662.6 & \Rc & 480.0 & $> 21.3$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,061222A & 2006 Dec 22.1496 & 424.8 & \Rc & 60.0 & $> 21.6$ \\
  $\cdots$ & 2006 Dec 22.1506 & 512.9 & \ip & 60.0 & $> 21.3$ \\
  $\cdots$ & 2006 Dec 22.1517 & 607.7 & \zp & 60.0 & $> 20.8$ \\
  $\cdots$ & 2006 Dec 22.1522 & 705.7 & \Rc & 180.0 & $> 22.3$ \\
  $\cdots$ & 2006 Dec 22.1532 & 797.5 & \ip & 180.0 & $> 22.2$ \\
  $\cdots$ & 2006 Dec 22.1543 & 893.7 & \zp & 180.0 & $> 21.3$ \\
  $\cdots$ & 2006 Dec 22.1649 & 1774.4 & \gG & 120.0 & $> 21.8$ \\ 
  $\cdots$ & 2006 Dec 22.1654 & 1934.3 & \Rc & 360.0 & $> 22.4$ \\
  $\cdots$ & 2006 Dec 22.1672 & 2090.3 & \ip & 360.0 & $> 22.2$ \\
  $\cdots$ & 2006 Dec 22.1690 & 2248.0 & \zp & 360.0 & $> 21.5$ \\
  $\cdots$ & 2006 Dec 22.1708 & 2404.0 & \gG & 360.0 & $> 22.1$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,070208 & 2007 Feb 8.3858 & 329.6 & \Rc & 60.0 & $19.27 \pm 0.06$ \\
  $\cdots$ & 2007 Feb 8.3875 & 475.5 & \ip & 60.0 & $19.17 \pm 0.04$ \\
  $\cdots$ & 2007 Feb 8.3887 & 583.2 & \zp & 60.0 & $18.76 \pm 0.10$ \\
  $\cdots$ & 2007 Feb 8.3901 & 697.7 & \Rc & 60.0 & $19.55 \pm 0.11$ \\
  $\cdots$ & 2007 Feb 8.3913 & 805.5 & \ip & 60.0 & $19.55 \pm 0.06$ \\
  $\cdots$ & 2007 Feb 8.3926 & 917.2 & \zp & 60.0 & $19.15 \pm 0.12$ \\
  $\cdots$ & 2007 Feb 8.3938 & 1022.6 & \Rc & 60.0 & $19.80 \pm 0.08$ \\
  $\cdots$ & 2007 Feb 8.3950 & 1127.5 & \ip & 60.0 & $19.65 \pm 0.06$ \\
  $\cdots$ & 2007 Feb 8.3963 & 1234.2 & \zp & 60.0 & $19.40 \pm 0.12$ \\
  $\cdots$ & 2007 Feb 8.3975 & 1371.5 & \Rc & 120.0 & $19.92 \pm 0.08$ \\
  $\cdots$ & 2007 Feb 8.3996 & 1554.0 & \ip & 120.0 & $19.82 \pm 0.09$ \\
  $\cdots$ & 2007 Feb 8.4038 & 1918.2 & \gG & 120.0 & $21.26 \pm 0.19$ \\
  $\cdots$ & 2007 Feb 8.4053 & 2104.3 & \zp & 240.0 & $19.61 \pm 0.10$ \\
  $\cdots$ & 2007 Feb 8.4060 & 2106.1 & \Rc & 120.0 & $20.13 \pm 0.17$ \\
  $\cdots$ & 2007 Feb 8.4081 & 2286.7 & \ip & 120.0 & $20.02 \pm 0.08$ \\
  $\cdots$ & 2007 Feb 8.4126 & 2673.1 & \gG & 120.0 & $21.67 \pm 0.22$ \\
  $\cdots$ & 2007 Feb 8.4161 & 2946.7 & \ip & 60.0 & $20.14 \pm 0.08$ \\
  $\cdots$ & 2007 Feb 8.4164 & 3001.4 & \Rc & 120.0 & $20.46 \pm 0.09$ \\
  $\cdots$ & 2007 Feb 8.4189 & 3218.0 & \zp & 120.0 & $19.54 \pm 0.11$ \\
  $\cdots$ & 2007 Feb 8.4198 & 3269.7 & \ip & 60.0 & $20.48 \pm 0.17$ \\
  $\cdots$ & 2007 Feb 8.4245 & 3700.7 & \ip & 120.0 & $20.26 \pm 0.09$ \\
  $\cdots$ & 2007 Feb 8.4329 & 4429.7 & \ip & 120.0 & $20.35 \pm 0.10$ \\
  $\cdots$ & 2007 Feb 8.4338 & 4625.5 & \zp & 360.0 & $20.53 \pm 0.15$ \\
  $\cdots$ & 2007 Feb 8.4359 & 4808.5 & \gG & 360.0 & $21.44 \pm 0.16$ \\
  $\cdots$ & 2007 Feb 8.4364 & 4853.9 & \Rc & 360.0 & $20.60 \pm 0.08$ \\
  $\cdots$ & 2007 Feb 8.4416 & 5177.7 & \ip & 120.0 & $20.57 \pm 0.12$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,070419A & 2007 Apr 19.4200 & 352.7 & \Rc & 60.0 & $19.52 \pm 0.13$ \\
  $\cdots$ & 2007 Apr 19.4212 & 454.7 & \ip & 60.0 & $18.71 \pm 0.05$ \\
  $\cdots$ & 2007 Apr 19.4224 & 560.8 & \zp & 60.0 & $18.12 \pm 0.09$ \\
  $\cdots$ & 2007 Apr 19.4236 & 665.9 & \Rc & 60.0 & $18.68 \pm 0.07$ \\
  $\cdots$ & 2007 Apr 19.4248 & 766.9 & \ip & 60.0 & $18.66 \pm 0.05$ \\
  $\cdots$ & 2007 Apr 19.4260 & 872.0 & \zp & 60.0 & $18.43 \pm 0.11$ \\
  $\cdots$ & 2007 Apr 19.4272 & 976.0 & \Rc & 60.0 & $19.09 \pm 0.12$ \\
  $\cdots$ & 2007 Apr 19.4284 & 1081.4 & \ip & 60.0 & $18.98 \pm 0.07$ \\
  $\cdots$ & 2007 Apr 19.4297 & 1189.0 & \zp & 60.0 & $18.58 \pm 0.10$ \\
  $\cdots$ & 2007 Apr 19.4309 & 1324.9 & \Rc & 120.0 & $19.22 \pm 0.08$ \\
  $\cdots$ & 2007 Apr 19.4330 & 1501.3 & \ip & 120.0 & $19.17 \pm 0.06$ \\
  $\cdots$ & 2007 Apr 19.4352 & 1691.3 & \zp & 120.0 & $19.56 \pm 0.18$ \\
  $\cdots$ & 2007 Apr 19.4393 & 2047.7 & \Rc & 120.0 & $19.75 \pm 0.12$ \\
  $\cdots$ & 2007 Apr 19.4413 & 2225.1 & \ip & 120.0 & $20.03 \pm 0.11$ \\
  $\cdots$ & 2007 Apr 19.4435 & 2408.2 & \zp & 120.0 & $19.52 \pm 0.20$ \\
  $\cdots$ & 2007 Apr 19.4443 & 2603.5 & \gG & 360.0 & $20.82 \pm 0.18$ \\
  $\cdots$ & 2007 Apr 19.4478 & 2787.5 & \Rc & 120.0 & $20.26 \pm 0.19$ \\
  $\cdots$ & 2007 Apr 19.4499 & 2966.1 & \ip & 120.0 & $20.36 \pm 0.16$ \\
  $\cdots$ & 2007 Apr 19.4521 & 3152.6 & \zp & 120.0 & $19.91 \pm 0.26$ \\
  $\cdots$ & 2007 Apr 19.4598 & 3944.6 & \Rc & 360.0 & $20.95 \pm 0.24$ \\
  $\cdots$ & 2007 Apr 19.4731 & 5271.5 & \ip & 720.0 & $21.01 \pm 0.15$ \\
  $\cdots$ & 2007 Apr 19.4783 & 5541.4 & \Rc & 360.0 & $21.33 \pm 0.38$ \\
  $\cdots$ & 2007 Apr 19.4793 & 5807.1 & \gG & 720.0 & $> 21.6$ \\
  $\cdots$ & 2007 Apr 20.2267 & $7.116 \times 10^{4}$ & \Rc & 2280.0 &
     $> 22.7$ \\
  $\cdots$ & 2007 Apr 20.2274 & $7.116 \times 10^{4}$ & \ip & 2160.0 &
     $> 22.7$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,070521 & 2007 May 21.2875 & 203.6 & \Rc & 60.0 & $> 21.6$ \\
  $\cdots$ & 2007 May 21.2886 & 296.4 & \ip & 60.0 & $> 21.5$ \\
  $\cdots$ & 2007 May 21.2897 & 390.0 & \zp & 60.0 & $> 20.5$ \\
  $\cdots$ & 2007 May 21.2901 & 487.2 & \Rc & 180.0 & $> 22.4$ \\
  $\cdots$ & 2007 May 21.2912 & 581.1 & \ip & 180.0 & $> 22.3$ \\
  $\cdots$ & 2007 May 21.2966 & 1106.3 & \zp & 300.0 & $> 21.3$ \\
  $\cdots$ & 2007 May 21.3142 & 2536.9 & \gG & 120.0 & $> 22.8$ \\
  $\cdots$ & 2007 May 21.3153 & 2695.0 & \zp & 240.0 & $> 21.3$ \\
  $\cdots$ & 2007 May 21.3147 & 2700.3 & \Rc & 360.0 & $> 23.0$ \\
  $\cdots$ & 2007 May 21.3166 & 2860.0 & \ip & 360.0 & $> 22.8$ \\
  $\cdots$ & 2007 May 21.3173 & 2865.2 & \gG & 240.0 & $> 23.3$ \\
  $\cdots$ & 2007 May 21.3400 & 9202.4 & \ip & 9000.0 & $> 23.6$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,071003\tablenotemark{e} & 2007 Oct 3.3221 & 206.0 & \Rc & 
     60.0 & $14.57 \pm 0.06$ \\
  $\cdots$ & 2007 Oct 3.3231 & 291.0 & \ip & 60.0 & $15.08 \pm 0.05$ \\
  $\cdots$ & 2007 Oct 3.3241 & 377.0 & \zp & 60.0 & $15.37 \pm 0.07$ \\
  $\cdots$ & 2007 Oct 3.3251 & 462.0 & \Rc & 60.0 & $16.03 \pm 0.07$ \\
  $\cdots$ & 2007 Oct 3.3261 & 548.0 & \ip & 60.0 & $16.41 \pm 0.07$ \\
  $\cdots$ & 2007 Oct 3.3271 & 633.0 & \zp & 60.0 & $16.43 \pm 0.08$ \\
  $\cdots$ & 2007 Oct 3.3281 & 719.0 & \Rc & 60.0 & $16.88 \pm 0.09$ \\
  $\cdots$ & 2007 Oct 3.3291 & 805.0 & \ip & 60.0 & $17.12 \pm 0.10$ \\
  $\cdots$ & 2007 Oct 3.3300 & 890.0 & \zp & 60.0 & $17.02 \pm 0.11$ \\
  $\cdots$ & 2007 Oct 3.3352 & 1369.0 & \zp & 120.0 & $17.92 \pm 0.20$ \\
  $\cdots$ & 2007 Oct 3.3369 & 1514.0 & \gG & 120.0 & $18.71 \pm 0.10$ \\
  $\cdots$ & 2007 Oct 3.3420 & 1951.0 & \zp & 120.0 & $18.67 \pm 0.28$ \\
  $\cdots$ & 2007 Oct 3.3437 & 2097.0 & \gG & 120.0 & $19.33 \pm 0.15$ \\
  $\cdots$ & 2007 Oct 3.3504 & 2678.0 & \gG & 120.0 & $19.44 \pm 0.20$ \\ 
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,071010A & 2007 Oct 10.1567 & 298.3 & \Rc & 60.0 & $16.37 \pm 0.21$ \\
  $\cdots$ & 2007 Oct 10.1577 & 383.8 & \ip & 60.0 & $16.42 \pm 0.17$ \\
  $\cdots$ & 2007 Oct 10.1587 & 469.4 & \zp & 60.0 & $16.50 \pm 0.37$ \\
  $\cdots$ & 2007 Oct 10.1597 & 554.9 & \Rc & 60.0 & $16.17 \pm 0.20$ \\
  $\cdots$ & 2007 Oct 10.1607 & 640.5 & \ip & 60.0 & $16.56 \pm 0.18$ \\
  $\cdots$ & 2007 Oct 10.1617 & 726.0 & \zp & 60.0 & $16.67 \pm 0.36$ \\
  $\cdots$ & 2007 Oct 10.1627 & 811.6 & \Rc & 60.0 & $16.44 \pm 0.19$ \\
  $\cdots$ & 2007 Oct 10.1637 & 897.4 & \ip & 60.0 & $16.86 \pm 0.18$ \\
  $\cdots$ & 2007 Oct 10.1646 & 982.9 & \zp & 60.0 & $17.29 \pm 0.29$ \\
  $\cdots$ & 2007 Oct 11.1234 & $8.469 \times 10^{4}$ & \Rc & 1800.0 & 
     $19.71 \pm 0.21$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,071011 & 2007 Oct 11.5303 & 235.3 & \Rc & 60.0 & $17.70 \pm 0.22$ \\
  $\cdots$ & 2007 Oct 11.5313 & 320.9 & \ip & 60.0 & $17.10 \pm 0.21$ \\
  $\cdots$ & 2007 Oct 11.5323 & 406.4 & \zp & 60.0 & $16.47 \pm 0.38$ \\
  $\cdots$ & 2007 Oct 11.5333 & 492.0 & \Rc & 60.0 & $18.17 \pm 0.27$ \\
  $\cdots$ & 2007 Oct 11.5343 & 577.7 & \ip & 60.0 & $17.67 \pm 0.24$ \\
  $\cdots$ & 2007 Oct 11.5353 & 663.2 & \zp & 60.0 & $17.09 \pm 0.31$ \\
  $\cdots$ & 2007 Oct 11.5362 & 748.8 & \Rc & 60.0 & $18.82 \pm 0.24$ \\
  $\cdots$ & 2007 Oct 11.5372 & 834.4 & \ip & 60.0 & $18.00 \pm 0.27$ \\
  $\cdots$ & 2007 Oct 11.5382 & 919.9 & \zp & 60.0 & $17.45 \pm 0.33$ \\
  $\cdots$ & 2007 Oct 12.2699 & $4.992 \times 10^{4}$ & \Rc & 1800.0 &
     $> 22.8$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,071020 & 2007 Oct 20.3461 & 4615.8 & \ip & 120.0 & $19.93 \pm 0.09$ \\
  $\cdots$ & 2007 Oct 20.3477 & 4753.8 & \ip & 120.0 & $19.88 \pm 0.08$ \\
  $\cdots$ & 2007 Oct 20.3493 & 4892.7 & \ip & 120.0 & $20.00 \pm 0.08$ \\
  $\cdots$ & 2007 Oct 20.3525 & 5169.1 & \Rc & 120.0 & $19.96 \pm 0.09$ \\
  $\cdots$ & 2007 Oct 20.3541 & 5307.3 & \Rc & 120.0 & $19.96 \pm 0.10$ \\
  $\cdots$ & 2007 Oct 20.3653 & 6276.9 & \ip & 120.0 & $20.00 \pm 0.08$ \\
  $\cdots$ & 2007 Oct 20.3669 & 6414.9 & \ip & 120.0 & $20.44 \pm 0.12$ \\
  $\cdots$ & 2007 Oct 20.3685 & 6553.0 & \ip & 120.0 & $20.20 \pm 0.10$ \\
  $\cdots$ & 2007 Oct 20.3541 & 5307.3 & \Rc & 120.0 & $19.96 \pm 0.10$ \\
  $\cdots$ & 2007 Oct 20.3559 & 5586.9 & \zp & 360.0 & $20.49 \pm 0.25$ \\
  $\cdots$ & 2007 Oct 20.3701 & 6691.3 & \Rc & 120.0 & $20.04 \pm 0.10$ \\
  $\cdots$ & 2007 Oct 20.3717 & 6829.3 & \Rc & 120.0 & $20.23 \pm 0.12$ \\
  $\cdots$ & 2007 Oct 20.3733 & 6967.5 & \Rc & 120.0 & $20.43 \pm 0.12$ \\
  $\cdots$ & 2007 Oct 20.3751 & 7246.9 & \zp & 360.0 & $19.96 \pm 0.14$ \\
  $\cdots$ & 2007 Oct 20.3845 & 7937.4 & \ip & 120.0 & $20.66 \pm 0.14$ \\
  $\cdots$ & 2007 Oct 20.3861 & 8075.4 & \ip & 120.0 & $20.32 \pm 0.10$ \\
  $\cdots$ & 2007 Oct 20.3877 & 8213.5 & \ip & 120.0 & $20.31 \pm 0.10$ \\
  $\cdots$ & 2007 Oct 20.3893 & 8351.6 & \Rc & 120.0 & $20.63 \pm 0.15$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,071122 & 2007 Nov 22.0709 & 1302.5 & \Rc & 360.0 & $20.22 \pm 0.22$ \\
  $\cdots$ & 2007 Nov 22.0760 & 1739.0 & \ip & 360.0 & $19.89 \pm 0.17$ \\
  $\cdots$ & 2007 Nov 22.0810 & 2175.5 & \zp & 360.0 & $19.71 \pm 0.39$ \\
  $\cdots$ & 2007 Nov 22.0997 & 3790.9 & \Rc & 360.0 & $19.89 \pm 0.20$ \\
  $\cdots$ & 2007 Nov 22.1048 & 4227.6 & \ip & 360.0 & $19.87 \pm 0.18$ \\
  $\cdots$ & 2007 Nov 22.1149 & 5101.3 & \Rc & 360.0 & $19.76 \pm 0.19$ \\
  $\cdots$ & 2007 Nov 22.1153 & 5319.5 & \zp & 720.0 & $19.69 \pm 0.38$ \\
  $\cdots$ & 2007 Nov 22.1199 & 5537.9 & \ip & 360.0 & $19.73 \pm 0.18$ \\
  $\cdots$ & 2007 Nov 22.1301 & 6416.3 & \Rc & 360.0 & $19.84 \pm 0.21$ \\
  $\cdots$ & 2007 Nov 22.1353 & 6863.0 & \ip & 360.0 & $19.82 \pm 0.18$ \\
  $\cdots$ & 2007 Nov 22.1454 & 7736.4 & \Rc & 360.0 & $19.77 \pm 0.21$ \\
  $\cdots$ & 2007 Nov 22.1458 & 7954.9 & \zp & 720.0 & $19.87 \pm 0.38$ \\
  $\cdots$ & 2007 Nov 22.1504 & 8173.4 & \ip & 360.0 & $19.87 \pm 0.19$ \\
  $\cdots$ & 2007 Nov 22.1606 & 9046.8 & \Rc & 360.0 & $20.11 \pm 0.22$ \\
  $\cdots$ & 2007 Nov 22.1656 & 9483.5 & \ip & 360.0 & $19.74 \pm 0.18$ \\
  $\cdots$ & 2007 Nov 23.0744 & $8.827 \times 10^{4}$ & \Rc & 900.0 &
     $> 20.8$ \\
  $\cdots$ & 2007 Nov 23.0783 & $8.843 \times 10^{4}$ & \ip & 540.0 & 
     $21.00 \pm 0.25$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,080310 & 2008 Mar 10.3628 & 298.3 & \Rc & 60.0 & $16.76 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 10.3638 & 384.0 & \ip & 60.0 & $16.87 \pm 0.11$ \\
  $\cdots$ & 2008 Mar 10.3648 & 470.2 & \zp & 60.0 & $16.76 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 10.3658 & 555.9 & \Rc & 60.0 & $17.04 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 10.3668 & 641.5 & \ip & 60.0 & $17.01 \pm 0.11$ \\
  $\cdots$ & 2008 Mar 10.3678 & 727.3 & \zp & 60.0 & $16.80 \pm 0.14$ \\
  $\cdots$ & 2008 Mar 10.3688 & 813.0 & \Rc & 60.0 & $17.05 \pm 0.20$ \\
  $\cdots$ & 2008 Mar 10.3698 & 898.7 & \ip & 60.0 & $16.98 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 10.3707 & 984.4 & \zp & 60.0 & $16.74 \pm 0.12$ \\
  $\cdots$ & 2008 Mar 10.3717 & 1100.3 & \Rc & 120.0 & $16.96 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 10.3734 & 1246.0 & \ip & 120.0 & $16.90 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 10.3751 & 1361.8 & \Rc & 60.0 & $16.91 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 10.3761 & 1447.5 & \ip & 60.0 & $16.92 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 10.3771 & 1533.4 & \zp & 60.0 & $16.70 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 10.3781 & 1619.3 & \Rc & 60.0 & $16.96 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 10.3791 & 1705.0 & \ip & 60.0 & $16.99 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 10.3801 & 1790.7 & \zp & 60.0 & $16.74 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 10.3811 & 1906.4 & \Rc & 120.0 & $16.98 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 10.3828 & 2052.3 & \ip & 120.0 & $17.02 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 10.3844 & 2198.1 & \zp & 120.0 & $16.91 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 10.3861 & 2343.8 & \gG & 120.0 & $17.86 \pm 0.13$ \\
  $\cdots$ & 2008 Mar 10.3878 & 2489.8 & \Rc & 120.0 & $17.15 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 10.3895 & 2635.6 & \ip & 120.0 & $17.21 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 10.3912 & 2781.4 & \zp & 120.0 & $17.10 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 10.3929 & 2927.1 & \gG & 120.0 & $18.00 \pm 0.12$ \\
  $\cdots$ & 2008 Mar 10.3946 & 3072.8 & \Rc & 120.0 & $17.30 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 10.3963 & 3218.6 & \ip & 120.0 & $17.35 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 10.3979 & 3364.3 & \zp & 120.0 & $17.24 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 10.3996 & 3510.1 & \gG & 120.0 & $18.12 \pm 0.12$ \\
  $\cdots$ & 2008 Mar 11.3202 & $8.325 \times 10^{4}$ & \ip & 540.0 & 
     $21.20 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 11.3273 & $8.387 \times 10^{4}$ & \Rc & 540.0 & 
     $21.36 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 11.3344 & $8.449 \times 10^{4}$ & \ip & 540.0 & 
     $21.22 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 11.3416 & $8.511 \times 10^{4}$ & \Rc & 540.0 & 
     $21.31 \pm 0.11$ \\
  $\cdots$ & 2008 Mar 11.3487 & $8.572 \times 10^{4}$ & \ip & 540.0 & 
     $21.40 \pm 0.24$ \\
  $\cdots$ & 2008 Mar 11.3559 & $8.634 \times 10^{4}$ & \Rc & 540.0 & 
     $21.17 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 11.3630 & $8.696 \times 10^{4}$ & \ip & 540.0 & 
     $21.32 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 11.3702 & $8.758 \times 10^{4}$ & \Rc & 540.0 & 
     $21.31 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 11.3814 & $8.882 \times 10^{4}$ & \ip & 1080.0 & 
     $21.19 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 11.3886 & $8.944 \times 10^{4}$ & \Rc & 1080.0 & 
     $21.39 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 11.4100 & $9.129 \times 10^{4}$ & \ip & 1080.0 & 
     $21.32 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 11.4172 & $9.190 \times 10^{4}$ & \Rc & 1080.0 & 
     $21.37 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 11.4386 & $9.376 \times 10^{4}$ & \ip & 1080.0 & 
     $21.29 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 11.4457 & $9.437 \times 10^{4}$ & \Rc & 1080.0 & 
     $21.37 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 13.3165 & $2.564 \times 10^{5}$ & \ip & 1800.0 &
     $> 21.7$ \\
  $\cdots$ & 2008 Mar 13.3403 & $2.584 \times 10^{5}$ & \Rc & 1800.0 & 
     $22.72 \pm 0.21$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,080319A & 2008 Mar 19.2417 & 173.5 & \Rc & 60.0 & $20.02 \pm 0.14$ \\
  $\cdots$ & 2008 Mar 19.2427 & 259.7 & \ip & 60.0 & $19.45 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.2437 & 346.0 & \zp & 60.0 & $19.03 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 19.2447 & 432.0 & \Rc & 60.0 & $19.71 \pm 0.11$ \\
  $\cdots$ & 2008 Mar 19.2457 & 518.0 & \ip & 60.0 & $19.67 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.2467 & 604.3 & \zp & 60.0 & $19.70 \pm 0.15$ \\
  $\cdots$ & 2008 Mar 19.2477 & 690.3 & \Rc & 60.0 & $20.18 \pm 0.17$ \\
  $\cdots$ & 2008 Mar 19.2487 & 776.4 & \ip & 60.0 & $20.20 \pm 0.12$ \\
  $\cdots$ & 2008 Mar 19.2497 & 862.5 & \zp & 60.0 & $19.40 \pm 0.13$ \\
  $\cdots$ & 2008 Mar 19.2508 & 983.6 & \Rc & 120.0 & $20.46 \pm 0.16$ \\
  $\cdots$ & 2008 Mar 19.2533 & 1231.8 & \Rc & 180.0 & $20.57 \pm 0.14$ \\
  $\cdots$ & 2008 Mar 19.2568 & 1507.0 & \Rc & 120.0 & $21.30 \pm 0.25$ \\
  $\cdots$ & 2008 Mar 19.2577 & 1550.1 & \zp & 60.0 & $20.39 \pm 0.27$ \\
  $\cdots$ & 2008 Mar 19.2578 & 1593.0 & \ip & 120.0 & $20.81 \pm 0.12$ \\
  $\cdots$ & 2008 Mar 19.2910 & 4462.1 & \Rc & 120.0 & $21.41 \pm 0.30$ \\
  $\cdots$ & 2008 Mar 19.2927 & 4607.8 & \ip & 120.0 & $21.38 \pm 0.21$ \\
  $\cdots$ & 2008 Mar 19.2944 & 4753.5 & \zp & 120.0 & $> 20.5$ \\
  $\cdots$ & 2008 Mar 20.2489 & $8.806 \times 10^{4}$ & \Rc & 1800.0 &
     $> 22.0$ \\
  $\cdots$ & 2008 Mar 20.2891 & $9.154 \times 10^{4}$ & \ip & 1800.0 &
     $> 22.3$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,080319B & 2008 Mar 19.2607 & 185.6 & \Rc & 60.0 & $< 11.13$ \\
  $\cdots$ & 2008 Mar 19.2617 & 271.9 & \ip & 60.0 & $11.55 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.2627 & 358.1 & \zp & 60.0 & $11.51 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 19.2637 & 444.2 & \Rc & 60.0 & $< 12.15$ \\
  $\cdots$ & 2008 Mar 19.2647 & 530.3 & \ip & 60.0 & $12.59 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.2657 & 616.6 & \zp & 60.0 & $12.65 \pm 0.26$ \\
  $\cdots$ & 2008 Mar 19.2667 & 702.8 & \Rc & 60.0 & $13.01 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.2677 & 788.7 & \ip & 60.0 & $13.33 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.2687 & 874.6 & \zp & 60.0 & $13.40 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.2697 & 990.4 & \Rc & 120.0 & $13.70 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.2714 & 1136.1 & \ip & 120.0 & $14.04 \pm 0.13$ \\
  $\cdots$ & 2008 Mar 19.2731 & 1287.0 & \zp & 120.0 & $14.22 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.2748 & 1432.7 & \gG & 120.0 & $15.13 \pm 0.20$ \\
  $\cdots$ & 2008 Mar 19.2765 & 1578.7 & \Rc & 120.0 & $14.68 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 19.2782 & 1724.5 & \ip & 120.0 & $14.99 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.2799 & 1870.3 & \zp & 120.0 & $15.01 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.2815 & 2016.1 & \gG & 120.0 & $15.77 \pm 0.21$ \\
  $\cdots$ & 2008 Mar 19.2832 & 2161.8 & \Rc & 120.0 & $15.29 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.2849 & 2307.6 & \ip & 120.0 & $15.51 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.2866 & 2453.3 & \zp & 120.0 & $15.47 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.2883 & 2599.1 & \gG & 120.0 & $16.14 \pm 0.17$ \\
  $\cdots$ & 2008 Mar 19.2970 & 3319.4 & \Rc & 60.0 & $15.93 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.2979 & 3397.6 & \ip & 60.0 & $16.09 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.2988 & 3476.3 & \zp & 60.0 & $16.02 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.2997 & 3558.2 & \Rc & 60.0 & $16.01 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3006 & 3636.5 & \ip & 60.0 & $16.18 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3015 & 3714.7 & \zp & 60.0 & $16.12 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3025 & 3796.1 & \Rc & 60.0 & $16.11 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3034 & 3874.3 & \ip & 60.0 & $16.27 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3043 & 3952.8 & \zp & 60.0 & $16.23 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3052 & 4034.6 & \Rc & 60.0 & $16.19 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3062 & 4112.8 & \ip & 60.0 & $16.34 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3071 & 4191.1 & \zp & 60.0 & $16.27 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3080 & 4272.6 & \Rc & 60.0 & $16.27 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3089 & 4351.1 & \ip & 60.0 & $16.41 \pm 0.02$ \\
  $\cdots$ & 2008 Mar 19.3098 & 4429.3 & \zp & 60.0 & $16.33 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3108 & 4511.1 & \Rc & 60.0 & $16.32 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3117 & 4589.4 & \ip & 60.0 & $16.49 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3126 & 4667.7 & \zp & 60.0 & $16.42 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3135 & 4749.3 & \Rc & 60.0 & $16.39 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3144 & 4827.6 & \ip & 60.0 & $16.55 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3153 & 4905.8 & \zp & 60.0 & $16.48 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3163 & 4987.2 & \Rc & 60.0 & $16.49 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3172 & 5065.6 & \ip & 60.0 & $16.61 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3181 & 5143.8 & \zp & 60.0 & $16.53 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3190 & 5225.4 & \Rc & 60.0 & $16.53 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3199 & 5303.6 & \ip & 60.0 & $16.69 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3208 & 5381.9 & \zp & 60.0 & $16.60 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3218 & 5463.4 & \Rc & 60.0 & $16.61 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3227 & 5541.7 & \ip & 60.0 & $16.74 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3236 & 5619.9 & \zp & 60.0 & $16.68 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3245 & 5701.8 & \Rc & 60.0 & $16.65 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3255 & 5780.2 & \ip & 60.0 & $16.81 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3264 & 5858.5 & \zp & 60.0 & $16.71 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3273 & 5940.0 & \Rc & 60.0 & $16.72 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3282 & 6018.3 & \ip & 60.0 & $16.84 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3291 & 6096.5 & \zp & 60.0 & $16.77 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3301 & 6178.3 & \Rc & 60.0 & $16.76 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3310 & 6256.7 & \ip & 60.0 & $16.90 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3319 & 6335.1 & \zp & 60.0 & $16.85 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3328 & 6416.6 & \Rc & 60.0 & $16.82 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3337 & 6494.8 & \ip & 60.0 & $16.95 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3346 & 6573.0 & \zp & 60.0 & $16.91 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3356 & 6654.9 & \Rc & 60.0 & $16.86 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3365 & 6733.1 & \ip & 60.0 & $16.98 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3374 & 6811.5 & \zp & 60.0 & $16.88 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3383 & 6892.9 & \Rc & 60.0 & $16.91 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3392 & 6971.2 & \ip & 60.0 & $17.05 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3401 & 7049.4 & \zp & 60.0 & $16.96 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3411 & 7131.0 & \Rc & 60.0 & $16.94 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3420 & 7209.3 & \ip & 60.0 & $17.09 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3429 & 7287.6 & \zp & 60.0 & $17.00 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3438 & 7368.9 & \Rc & 60.0 & $17.02 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3447 & 7447.2 & \ip & 60.0 & $17.13 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3457 & 7525.5 & \zp & 60.0 & $17.04 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3466 & 7607.1 & \Rc & 60.0 & $17.02 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3475 & 7685.5 & \ip & 60.0 & $17.18 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3484 & 7763.8 & \zp & 60.0 & $17.12 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3494 & 7845.3 & \Rc & 60.0 & $17.09 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3503 & 7923.7 & \ip & 60.0 & $17.21 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3512 & 8002.4 & \zp & 60.0 & $17.12 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3521 & 8084.1 & \Rc & 60.0 & $17.14 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3530 & 8162.5 & \ip & 60.0 & $17.25 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3539 & 8241.1 & \zp & 60.0 & $17.21 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3549 & 8322.8 & \Rc & 60.0 & $17.15 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3558 & 8401.1 & \ip & 60.0 & $17.30 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3567 & 8479.4 & \zp & 60.0 & $17.21 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3576 & 8560.9 & \Rc & 60.0 & $17.20 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3585 & 8639.2 & \ip & 60.0 & $17.34 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3595 & 8717.5 & \zp & 60.0 & $17.28 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3639 & 9105.0 & \Rc & 60.0 & $17.30 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3648 & 9183.3 & \ip & 60.0 & $17.41 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3657 & 9261.6 & \zp & 60.0 & $17.34 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3667 & 9342.8 & \Rc & 60.0 & $17.31 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3676 & 9422.1 & \ip & 60.0 & $17.45 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3685 & 9500.4 & \zp & 60.0 & $17.33 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3695 & 9581.9 & \Rc & 60.0 & $17.38 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3704 & 9660.1 & \ip & 60.0 & $17.47 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3713 & 9738.6 & \zp & 60.0 & $17.36 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3722 & 9820.1 & \Rc & 60.0 & $17.41 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3731 & 9898.3 & \ip & 60.0 & $17.48 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3740 & 9976.6 & \zp & 60.0 & $17.45 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3750 & $1.006 \times 10^{4}$ & \Rc & 60.0 & 
     $17.43 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3759 & $1.014 \times 10^{4}$ & \ip & 60.0 & 
     $17.52 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3768 & $1.021 \times 10^{4}$ & \zp & 60.0 & 
     $17.49 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3777 & $1.030 \times 10^{4}$ & \Rc & 60.0 & 
     $17.45 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3786 & $1.037 \times 10^{4}$ & \ip & 60.0 & 
     $17.60 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3795 & $1.045 \times 10^{4}$ & \zp & 60.0 & 
     $17.52 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3805 & $1.053 \times 10^{4}$ & \Rc & 60.0 & 
     $17.49 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.3814 & $1.061 \times 10^{4}$ & \ip & 60.0 & 
     $17.64 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3823 & $1.069 \times 10^{4}$ & \zp & 60.0 & 
     $17.53 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.3832 & $1.077 \times 10^{4}$ & \Rc & 60.0 & 
     $17.52 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 19.3841 & $1.085 \times 10^{4}$ & \ip & 60.0 & 
     $17.63 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3850 & $1.093 \times 10^{4}$ & \zp & 60.0 & 
     $17.54 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3860 & $1.101 \times 10^{4}$ & \Rc & 60.0 & 
     $17.57 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3869 & $1.109 \times 10^{4}$ & \ip & 60.0 & 
     $17.66 \pm 0.02$ \\
  $\cdots$ & 2008 Mar 19.3878 & $1.117 \times 10^{4}$ & \zp & 60.0 & 
     $17.57 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.3887 & $1.125 \times 10^{4}$ & \Rc & 60.0 & 
     $17.61 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3897 & $1.133 \times 10^{4}$ & \ip & 60.0 & 
     $17.70 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3906 & $1.141 \times 10^{4}$ & \zp & 60.0 & 
     $17.66 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.3915 & $1.149 \times 10^{4}$ & \Rc & 60.0 & 
     $17.61 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3924 & $1.156 \times 10^{4}$ & \ip & 60.0 & 
     $17.72 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.3933 & $1.164 \times 10^{4}$ & \zp & 60.0 & 
     $17.62 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3943 & $1.172 \times 10^{4}$ & \Rc & 60.0 & 
     $17.64 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3952 & $1.180 \times 10^{4}$ & \ip & 60.0 & 
     $17.76 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3961 & $1.188 \times 10^{4}$ & \zp & 60.0 & 
     $17.67 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3971 & $1.197 \times 10^{4}$ & \Rc & 60.0 & 
     $17.67 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.3980 & $1.205 \times 10^{4}$ & \ip & 60.0 & 
     $17.78 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.3989 & $1.212 \times 10^{4}$ & \zp & 60.0 & 
     $17.71 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.3998 & $1.221 \times 10^{4}$ & \Rc & 60.0 & 
     $17.70 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4007 & $1.228 \times 10^{4}$ & \ip & 60.0 & 
     $17.81 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4016 & $1.236 \times 10^{4}$ & \zp & 60.0 & 
     $17.68 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4026 & $1.244 \times 10^{4}$ & \Rc & 60.0 & 
     $17.69 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4035 & $1.252 \times 10^{4}$ & \ip & 60.0 & 
     $17.82 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4044 & $1.260 \times 10^{4}$ & \zp & 60.0 & 
     $17.72 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4053 & $1.268 \times 10^{4}$ & \Rc & 60.0 & 
     $17.75 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4062 & $1.276 \times 10^{4}$ & \ip & 60.0 & 
     $17.85 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4071 & $1.284 \times 10^{4}$ & \zp & 60.0 & 
     $17.71 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4081 & $1.292 \times 10^{4}$ & \Rc & 60.0 & 
     $17.78 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4090 & $1.300 \times 10^{4}$ & \ip & 60.0 & 
     $17.86 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4099 & $1.308 \times 10^{4}$ & \zp & 60.0 & 
     $17.74 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.4108 & $1.316 \times 10^{4}$ & \Rc & 60.0 & 
     $17.81 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4118 & $1.324 \times 10^{4}$ & \ip & 60.0 & 
     $17.91 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4127 & $1.331 \times 10^{4}$ & \zp & 60.0 & 
     $17.79 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4136 & $1.340 \times 10^{4}$ & \Rc & 60.0 & 
     $17.80 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4145 & $1.347 \times 10^{4}$ & \ip & 60.0 & 
     $17.90 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4154 & $1.355 \times 10^{4}$ & \zp & 60.0 & 
     $17.88 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4164 & $1.363 \times 10^{4}$ & \Rc & 60.0 & 
     $17.83 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4173 & $1.371 \times 10^{4}$ & \ip & 60.0 & 
     $17.94 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4182 & $1.379 \times 10^{4}$ & \zp & 60.0 & 
     $17.83 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4191 & $1.387 \times 10^{4}$ & \Rc & 60.0 & 
     $17.85 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4200 & $1.395 \times 10^{4}$ & \ip & 60.0 & 
     $17.95 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4209 & $1.403 \times 10^{4}$ & \zp & 60.0 & 
     $17.89 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.4219 & $1.411 \times 10^{4}$ & \Rc & 60.0 & 
     $17.84 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4228 & $1.419 \times 10^{4}$ & \ip & 60.0 & 
     $18.01 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4237 & $1.427 \times 10^{4}$ & \zp & 60.0 & 
     $17.93 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4246 & $1.435 \times 10^{4}$ & \Rc & 60.0 & 
     $17.92 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4256 & $1.443 \times 10^{4}$ & \ip & 60.0 & 
     $18.02 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4265 & $1.451 \times 10^{4}$ & \zp & 60.0 & 
     $17.87 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.4274 & $1.459 \times 10^{4}$ & \Rc & 60.0 & 
     $17.92 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4283 & $1.467 \times 10^{4}$ & \ip & 60.0 & 
     $18.04 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4293 & $1.475 \times 10^{4}$ & \zp & 60.0 & 
     $17.92 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4302 & $1.483 \times 10^{4}$ & \Rc & 60.0 & 
     $17.99 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4311 & $1.491 \times 10^{4}$ & \ip & 60.0 & 
     $18.07 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4320 & $1.499 \times 10^{4}$ & \zp & 60.0 & 
     $17.96 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4330 & $1.507 \times 10^{4}$ & \Rc & 60.0 & 
     $17.97 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4339 & $1.515 \times 10^{4}$ & \ip & 60.0 & 
     $18.05 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4348 & $1.523 \times 10^{4}$ & \zp & 60.0 & 
     $18.02 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4357 & $1.531 \times 10^{4}$ & \Rc & 60.0 & 
     $17.97 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4366 & $1.538 \times 10^{4}$ & \ip & 60.0 & 
     $18.10 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4375 & $1.546 \times 10^{4}$ & \zp & 60.0 & 
     $18.17 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4385 & $1.554 \times 10^{4}$ & \Rc & 60.0 & 
     $18.02 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4394 & $1.562 \times 10^{4}$ & \ip & 60.0 & 
     $18.07 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4403 & $1.570 \times 10^{4}$ & \zp & 60.0 & 
     $18.12 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4412 & $1.578 \times 10^{4}$ & \Rc & 60.0 & 
     $18.05 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 19.4421 & $1.586 \times 10^{4}$ & \ip & 60.0 & 
     $18.16 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4430 & $1.594 \times 10^{4}$ & \zp & 60.0 & 
     $18.02 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4440 & $1.602 \times 10^{4}$ & \Rc & 60.0 & 
     $18.07 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4449 & $1.610 \times 10^{4}$ & \ip & 60.0 & 
     $18.19 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4458 & $1.618 \times 10^{4}$ & \zp & 60.0 & 
     $18.12 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4467 & $1.626 \times 10^{4}$ & \Rc & 60.0 & 
     $18.11 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4476 & $1.634 \times 10^{4}$ & \ip & 60.0 & 
     $18.18 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4485 & $1.642 \times 10^{4}$ & \zp & 60.0 & 
     $18.09 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4495 & $1.650 \times 10^{4}$ & \Rc & 60.0 & 
     $18.09 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4504 & $1.658 \times 10^{4}$ & \ip & 60.0 & 
     $18.23 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4513 & $1.665 \times 10^{4}$ & \zp & 60.0 & 
     $18.13 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4522 & $1.673 \times 10^{4}$ & \Rc & 60.0 & 
     $18.16 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4532 & $1.681 \times 10^{4}$ & \ip & 60.0 & 
     $18.20 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4541 & $1.689 \times 10^{4}$ & \zp & 60.0 & 
     $18.02 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4550 & $1.697 \times 10^{4}$ & \Rc & 60.0 & 
     $18.11 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4559 & $1.705 \times 10^{4}$ & \ip & 60.0 & 
     $18.24 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4578 & $1.721 \times 10^{4}$ & \Rc & 60.0 & 
     $18.19 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4587 & $1.729 \times 10^{4}$ & \ip & 60.0 & 
     $18.32 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4596 & $1.737 \times 10^{4}$ & \zp & 60.0 & 
     $18.26 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4606 & $1.745 \times 10^{4}$ & \Rc & 60.0 & 
     $18.17 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4615 & $1.753 \times 10^{4}$ & \ip & 60.0 & 
     $18.28 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4624 & $1.761 \times 10^{4}$ & \zp & 60.0 & 
     $18.18 \pm 0.11$ \\
  $\cdots$ & 2008 Mar 19.4633 & $1.769 \times 10^{4}$ & \Rc & 60.0 & 
     $18.23 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4651 & $1.785 \times 10^{4}$ & \ip & 60.0 & 
     $18.30 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4660 & $1.793 \times 10^{4}$ & \zp & 60.0 & 
     $18.15 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4670 & $1.801 \times 10^{4}$ & \Rc & 60.0 & 
     $18.27 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4680 & $1.810 \times 10^{4}$ & \ip & 60.0 & 
     $18.36 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4690 & $1.819 \times 10^{4}$ & \zp & 60.0 & 
     $18.16 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4700 & $1.827 \times 10^{4}$ & \Rc & 60.0 & 
     $18.27 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.4709 & $1.835 \times 10^{4}$ & \ip & 60.0 & 
     $18.36 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4719 & $1.843 \times 10^{4}$ & \zp & 60.0 & 
     $18.11 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4728 & $1.851 \times 10^{4}$ & \Rc & 60.0 & 
     $18.24 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4737 & $1.859 \times 10^{4}$ & \ip & 60.0 & 
     $18.40 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4746 & $1.867 \times 10^{4}$ & \zp & 60.0 & 
     $18.30 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4756 & $1.875 \times 10^{4}$ & \Rc & 60.0 & 
     $18.27 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4765 & $1.883 \times 10^{4}$ & \ip & 60.0 & 
     $18.39 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4774 & $1.891 \times 10^{4}$ & \zp & 60.0 & 
     $18.31 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4783 & $1.899 \times 10^{4}$ & \Rc & 60.0 & 
     $18.31 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4792 & $1.907 \times 10^{4}$ & \ip & 60.0 & 
     $18.44 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4801 & $1.914 \times 10^{4}$ & \zp & 60.0 & 
     $18.28 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4811 & $1.923 \times 10^{4}$ & \Rc & 60.0 & 
     $18.34 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4820 & $1.930 \times 10^{4}$ & \ip & 60.0 & 
     $18.39 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4829 & $1.938 \times 10^{4}$ & \zp & 60.0 & 
     $18.23 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4838 & $1.946 \times 10^{4}$ & \Rc & 60.0 & 
     $18.38 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4847 & $1.954 \times 10^{4}$ & \ip & 60.0 & 
     $18.46 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4856 & $1.962 \times 10^{4}$ & \zp & 60.0 & 
     $18.33 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4866 & $1.970 \times 10^{4}$ & \Rc & 60.0 & 
     $18.38 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4875 & $1.978 \times 10^{4}$ & \ip & 60.0 & 
     $18.45 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4884 & $1.986 \times 10^{4}$ & \zp & 60.0 & 
     $18.33 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.4893 & $1.994 \times 10^{4}$ & \Rc & 60.0 & 
     $18.29 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.4902 & $2.002 \times 10^{4}$ & \ip & 60.0 & 
     $18.46 \pm 0.03$ \\
  $\cdots$ & 2008 Mar 19.4912 & $2.010 \times 10^{4}$ & \zp & 60.0 & 
     $18.38 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4921 & $2.018 \times 10^{4}$ & \Rc & 60.0 & 
     $18.38 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4930 & $2.026 \times 10^{4}$ & \ip & 60.0 & 
     $18.49 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.4939 & $2.033 \times 10^{4}$ & \zp & 60.0 & 
     $18.41 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4949 & $2.042 \times 10^{4}$ & \Rc & 60.0 & 
     $18.39 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4958 & $2.049 \times 10^{4}$ & \ip & 60.0 & 
     $18.52 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4967 & $2.057 \times 10^{4}$ & \zp & 60.0 & 
     $18.34 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 19.4976 & $2.065 \times 10^{4}$ & \Rc & 60.0 & 
     $18.39 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.4985 & $2.073 \times 10^{4}$ & \ip & 60.0 & 
     $18.54 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.4994 & $2.081 \times 10^{4}$ & \zp & 60.0 & 
     $18.32 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.5004 & $2.089 \times 10^{4}$ & \Rc & 60.0 & 
     $18.45 \pm 0.06$ \\ 
  $\cdots$ & 2008 Mar 19.5013 & $2.097 \times 10^{4}$ & \ip & 60.0 & 
     $18.50 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.5022 & $2.105 \times 10^{4}$ & \zp & 60.0 & 
     $18.45 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.5031 & $2.113 \times 10^{4}$ & \Rc & 60.0 & 
     $18.42 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.5040 & $2.121 \times 10^{4}$ & \ip & 60.0 & 
     $18.53 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.5049 & $2.129 \times 10^{4}$ & \zp & 60.0 & 
     $18.31 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.5059 & $2.137 \times 10^{4}$ & \Rc & 60.0 & 
     $18.44 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.5068 & $2.145 \times 10^{4}$ & \ip & 60.0 & 
     $18.54 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.5077 & $2.153 \times 10^{4}$ & \zp & 60.0 & 
     $18.38 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 19.5086 & $2.161 \times 10^{4}$ & \Rc & 60.0 & 
     $18.45 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.5095 & $2.169 \times 10^{4}$ & \ip & 60.0 & 
     $18.61 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.5105 & $2.176 \times 10^{4}$ & \zp & 60.0 & 
     $18.50 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.5114 & $2.185 \times 10^{4}$ & \Rc & 60.0 & 
     $18.44 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.5123 & $2.192 \times 10^{4}$ & \ip & 60.0 & 
     $18.51 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.5132 & $2.200 \times 10^{4}$ & \zp & 60.0 & 
     $18.46 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.5142 & $2.208 \times 10^{4}$ & \Rc & 60.0 & 
     $18.45 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.5151 & $2.216 \times 10^{4}$ & \ip & 60.0 & 
     $18.59 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.5160 & $2.224 \times 10^{4}$ & \zp & 60.0 & 
     $18.45 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 19.5169 & $2.232 \times 10^{4}$ & \Rc & 60.0 & 
     $18.49 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.5179 & $2.241 \times 10^{4}$ & \ip & 60.0 & 
     $18.60 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.5188 & $2.248 \times 10^{4}$ & \zp & 60.0 & 
     $18.49 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.5197 & $2.257 \times 10^{4}$ & \Rc & 60.0 & 
     $18.57 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.5206 & $2.264 \times 10^{4}$ & \ip & 60.0 & 
     $18.66 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.5215 & $2.272 \times 10^{4}$ & \zp & 60.0 & 
     $18.52 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 19.5225 & $2.280 \times 10^{4}$ & \Rc & 60.0 & 
     $18.60 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.5234 & $2.288 \times 10^{4}$ & \ip & 60.0 & 
     $18.67 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.5243 & $2.296 \times 10^{4}$ & \zp & 60.0 & 
     $18.57 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 19.5252 & $2.304 \times 10^{4}$ & \Rc & 60.0 & 
     $18.57 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.5261 & $2.312 \times 10^{4}$ & \ip & 60.0 & 
     $18.65 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.5270 & $2.320 \times 10^{4}$ & \zp & 60.0 & 
     $18.62 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 19.5280 & $2.328 \times 10^{4}$ & \Rc & 60.0 & 
     $18.54 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 19.5289 & $2.336 \times 10^{4}$ & \ip & 60.0 & 
     $18.69 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.5298 & $2.344 \times 10^{4}$ & \zp & 60.0 & 
     $18.47 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 19.5307 & $2.352 \times 10^{4}$ & \Rc & 60.0 & 
     $18.53 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 20.2329 & $8.442 \times 10^{4}$ & \Rc & 540.0 & 
     $20.08 \pm 0.16$ \\
  $\cdots$ & 2008 Mar 20.2397 & $8.501 \times 10^{4}$ & \ip & 540.0 & 
     $20.17 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 20.2692 & $8.756 \times 10^{4}$ & \Rc & 540.0 & 
     $20.02 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 20.2761 & $8.816 \times 10^{4}$ & \ip & 540.0 & 
     $20.24 \pm 0.07$ \\
  $\cdots$ & 2008 Mar 20.3056 & $9.070 \times 10^{4}$ & \Rc & 540.0 & 
     $19.97 \pm 0.17$ \\
  $\cdots$ & 2008 Mar 20.3125 & $9.130 \times 10^{4}$ & \ip & 540.0 & 
     $20.46 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 20.3432 & $9.396 \times 10^{4}$ & \Rc & 540.0 & 
     $20.36 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 20.3501 & $9.455 \times 10^{4}$ & \ip & 540.0 & 
     $20.62 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 20.3795 & $9.709 \times 10^{4}$ & \Rc & 540.0 & 
     $20.73 \pm 0.12$ \\
  $\cdots$ & 2008 Mar 20.3864 & $9.769 \times 10^{4}$ & \ip & 540.0 & 
     $20.73 \pm 0.13$ \\
  $\cdots$ & 2008 Mar 20.4164 & $1.003 \times 10^{5}$ & \Rc & 540.0 & 
     $20.59 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 20.4233 & $1.009 \times 10^{5}$ & \ip & 540.0 & 
     $20.58 \pm 0.06$ \\
  $\cdots$ & 2008 Mar 20.4533 & $1.035 \times 10^{5}$ & \Rc & 540.0 & 
     $20.37 \pm 0.09$ \\
  $\cdots$ & 2008 Mar 20.4602 & $1.041 \times 10^{5}$ & \ip & 540.0 & 
     $20.55 \pm 0.08$ \\
  $\cdots$ & 2008 Mar 21.2315 & $1.712 \times 10^{5}$ & \Rc & 1620.0 & 
     $20.99 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 21.2534 & $1.731 \times 10^{5}$ & \ip & 1620.0 & 
     $21.32 \pm 0.11$ \\
  $\cdots$ & 2008 Mar 21.4043 & $1.863 \times 10^{5}$ & \Rc & 1800.0 & 
     $21.58 \pm 0.12$ \\
  $\cdots$ & 2008 Mar 21.4273 & $1.882 \times 10^{5}$ & \ip & 1800.0 & 
     $21.66 \pm 0.12$ \\
  $\cdots$ & 2008 Mar 22.4094 & $2.749 \times 10^{5}$ & \Rc & 5400.0 & 
     $21.90 \pm 0.11$ \\
  $\cdots$ & 2008 Mar 22.4324 & $2.769 \times 10^{5}$ & \ip & 5400.0 & 
     $22.21 \pm 0.10$ \\
  $\cdots$ & 2008 Mar 24.2450 & $4.335 \times 10^{5}$ & \Rc & 5400.0 & 
     $22.84 \pm 0.27$ \\
  $\cdots$ & 2008 Mar 24.2679 & $4.355 \times 10^{5}$ & \ip & 5400.0 & 
     $22.48 \pm 0.14$ \\
  $\cdots$ & 2008 Mar 25.2842 & $5.233 \times 10^{5}$ & \Rc & 5400.0 & 
     $22.73 \pm 0.19$ \\
  $\cdots$ & 2008 Mar 25.3072 & $5.253 \times 10^{5}$ & \ip & 5400.0 & 
     $22.92 \pm 0.17$ \\
  $\cdots$ & 2008 Mar 26.2822 & $6.095 \times 10^{5}$ & \Rc & 5400.0 & 
     $22.89 \pm 0.18$ \\
  $\cdots$ & 2008 Mar 26.3051 & $6.115 \times 10^{5}$ & \ip & 5400.0 & 
     $22.72 \pm 0.12$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,080319C & 2008 Mar 19.5321 & 1243.3 & \Rc & 60.0 & $18.66 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.5330 & 1329.0 & \ip & 60.0 & $18.51 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.5340 & 1414.9 & \zp & 60.0 & $18.19 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.5350 & 1500.7 & \Rc & 60.0 & $19.02 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 19.5360 & 1586.6 & \ip & 60.0 & $18.74 \pm 0.04$ \\
  $\cdots$ & 2008 Mar 19.5370 & 1672.4 & \zp & 60.0 & $18.41 \pm 0.05$ \\
  $\cdots$ & 2008 Mar 20.3959 & $7.675 \times 10^{4}$ & \Rc & 1800.0 & 
     $> 22.0$ \\
  $\cdots$ & 2008 Mar 20.4367 & $8.027 \times 10^{4}$ & \ip & 1800.0 & 
     $22.24 \pm 0.18$ \\
  $\cdots$ & 2008 Mar 21.4372 & $1.667 \times 10^{5}$ & \ip & 1800.0 & 
     $22.54 \pm 0.18$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  GRB\,080320 & 2008 Mar 20.1963 & 329.9 & \Rc & 60.0 & $> 20.1$ \\
  $\cdots$ & 2008 Mar 20.1973 & 415.6 & \ip & 60.0 & $> 20.2$ \\ 
  $\cdots$ & 2008 Mar 20.1983 & 501.4 & \zp & 60.0 & $> 19.1$ \\
  $\cdots$ & 2008 Mar 20.2008 & 810.4 & \Rc & 300.0 & $> 21.0$ \\
  $\cdots$ & 2008 Mar 20.2014 & 896.2 & \ip & 300.0 & $> 20.9$ \\
  $\cdots$ & 2008 Mar 20.2027 & 974.6 & \zp & 240.0 & $20.06 \pm 0.21$ \\
  $\cdots$ & 2008 Mar 20.2153 & 2003.4 & \gG & 120.0 & $> 20.9$ \\
  $\cdots$ & 2008 Mar 20.2156 & 2149.0 & \Rc & 360.0 & $> 21.5$ \\
  $\cdots$ & 2008 Mar 20.2173 & 2294.8 & \ip & 360.0 & $21.62 \pm 0.25$ \\
  $\cdots$ & 2008 Mar 20.2190 & 2440.6 & \zp & 360.0 & $> 20.5$ \\
  \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  \enddata
  \tablenotetext{a}{UT at beginning of exposure.}
  \tablenotetext{b}{Time from mid-point of exposure to \Swift-BAT trigger.}
  \tablenotetext{c}{Reference: \citet{snc+07}}
  \tablenotetext{d}{Reference: \citet{ckh+06}}
  \tablenotetext{e}{Reference: \citet{plc+08}}
\label{tab:p60catalog}
\end{deluxetable}

%\end{input}


==> tab2.tex <==
\ProvidesFile{p60filters.tab.tex}

\begin{deluxetable}{ccccc}
  \tabletypesize{\footnotesize}
  \tablecaption{P60 Filter Reference}
  \tablecolumns{5}
  \tablewidth{0pc}
  \tablehead{\colhead{P60 Filter} & \colhead{Central 
             Wavelength\tablenotemark{a}} & \colhead{Reference Filter} & 
             \colhead{Photometric System} & 
             \colhead{Zeropoint\tablenotemark{a}} \\
             & \colhead{(\AA)} & & & \colhead{(Jy)}
            }
  \startdata
  \gG & 4927 & \gp & AB & 3631 \\
  \Vc & 5505 & \Vc & Vega & 3590 \\
  \Rc & 6588 & \Rc & Vega & 3020 \\
  \ip & 7706 & \ip & AB & 3631 \\
  \iG & 7973 & \Ic & Vega & 2380 \\
  \Ic & 8060 & \Ic & Vega & 2380 \\
  \zG & 9133 & \zp & AB & 3631 \\
  \zp & 9222 & \zp & AB & 3631 \\
  \enddata
  \tablenotetext{a}{Reference: \citet{fsi95}.}
\label{tab:p60filters}
\end{deluxetable}


==> tab3.tex <==
\ProvidesFile{earlyafterglows.tab.tex}

\begin{landscape}
\begin{deluxetable}{lcccccccccc}
  \tabletypesize{\tiny}
  \tablecaption{P60-\Swift\ Early Optical Afterglow Sample}
  \tablecolumns{11}
  \tablewidth{0pc}
  \tablehead{\colhead{GRB Name} & \colhead{P60 OT?} & 
             \colhead{Other OT/IRT?\tablenotemark{a}} & 
             \colhead{Redshift\tablenotemark{b}} & 
             \colhead{$\alpha_{1}$\tablenotemark{c}} & 
             \colhead{$\alpha_{2}$\tablenotemark{c}} & 
             \colhead{$t_{b}$\tablenotemark{c}} &
             \colhead{$\beta_{\mathrm{O}}$\tablenotemark{c}}
             & \colhead{$\chi^{2}_{\mathrm{r}}$ (d.o.f.)\tablenotemark{c}} & 
             \colhead{$\beta_{OX}$\tablenotemark{d}} & 
             \colhead{$A_{V}$(host)\tablenotemark{e}} \\  
             & & & & & & \colhead{($10^{3}$\,s)} & & & & \colhead{(mag)} \\
            }
  \startdata
  050412 & No & No & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ &
    $\cdots$ & $< 0.49$ & $\cdots$ \\
  050416A & Yes & $\cdots$ & 0.6535 & $0.23 \pm 0.08$ & $0.9_{-0.3}^{+2.0}$ & 
    $11.6_{-8.9}^{+66.6}$ & $2.6 \pm 1.8$ & 1.33 (7) & 0.35 & $\cdots$ \\ 
  050607 & No & OT & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ &
    $\cdots$ & $< 0.72$ & $\cdots$ \\
  050713A & Yes & $\cdots$ & $\cdots$ & $0.62_{-0.11}^{+0.12}$ & $\cdots$ & 
    $\cdots$ & $\cdots$ & 0.72 (7) & 0.31 & $\cdots$ \\
  050820A\tablenotemark{f} & Yes & $\cdots$ & 2.615 & $\cdots$ & $\cdots$ & 
    $\cdots$ & $\cdots$ & $\cdots$ & 0.40 & $< 0.10$ \\
  050908 & Yes & $\cdots$ & 3.35 & $0.69 \pm 0.05$ & $\cdots$ & $\cdots$ &
    $-0.4 \pm 1.1$ & 0.75 (12) & 0.91 & $\cdots$ \\
  050915A & No & IRT & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ &
    $\cdots$ & $< 0.44$ & $\cdots$ \\
  060110 & Yes & $\cdots$ & $\cdots$ & $0.92_{-0.25}^{+0.30}$ & $\cdots$ & 
    $\cdots$ & $\cdots$ & 0.23 (8) & 0.80 & $\cdots$ \\
  060210 & Yes & $\cdots$ & 3.91 & $0.93 \pm 0.06$ & $\cdots$ & $\cdots$ & 
    $7.2 \pm 0.7$ & 1.43 (21) & 0.37 & $1.21_{-0.12}^{+0.16}$ \\
  060502A & Yes & $\cdots$ & 1.51 & $0.49 \pm 0.05$ & $\cdots$ & $\cdots$ &
    $2.1 \pm 0.3$ & 0.42 (24) & 0.53 & $0.53 \pm 0.13$ \\
  060510B & Yes & $\cdots$ & 4.9 & $0.3 \pm 0.5$ & $\cdots$ & $\cdots$ & 
    $4.2_{-2.2}^{+1.8}$ & 0.15 (4) & 0.04 & $\cdots$ \\
  060805A & No & No & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ &
    $\cdots$ & $< 0.76$ & $\cdots$ \\
  060906\tablenotemark{g} & Yes & $\cdots$ & 3.685 & $\cdots$ & $\cdots$ & 
    $\cdots$ & $2.2 \pm 0.2$ & 0.22 (20) & 0.88 & $0.20_{-0.12}^{+0.01}$ \\
  060908 & Yes & $\cdots$ & 2.43 & $1.04 \pm 0.02$ & $\cdots$ & $\cdots$ & 
    $0.59 \pm 0.07$ & 2.27 (52) & 0.82 & $\cdots$ \\
  060923A & No & IRT & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ &
    $\cdots$ & $< 0.41$ & $\cdots$ \\
  061222A & No & IRT & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ &
    $\cdots$ & $< 0.15$ & $\cdots$ \\
  070208 & Yes & $\cdots$ & 1.165 & $0.51 \pm 0.02$ & $\cdots$ & $\cdots$ & 
    $2.21 \pm 0.12$ & 1.65 (23) & 0.54 & $1.03 \pm 0.09$ \\
  070419A & Yes & $\cdots$ & 0.97 & $-1.6 \pm 0.3$ & $1.08 \pm 0.04$ & 
    $0.59 \pm 0.02$ & $1.8 \pm 0.2$ & 2.48 (16) & 0.87 & $1.03 \pm 0.17$ \\
  070521 & No & No & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ &
    $\cdots$ & $< -0.03$ & $\cdots$ \\
  071003 & Yes & $\cdots$ & 1.60435 & $1.77 \pm 0.05$ & $\cdots$ & $\cdots$ & 
    $0.86 \pm 0.19$ & 0.48 (8) & 0.27 & $< 0.26$ \\
  071010A & Yes & $\cdots$ & $\cdots$ & $0.29 \pm 0.19$ & $\cdots$ & $\cdots$ &
    $-1.1 \pm 0.7$ & 0.69 (6) & $0.89$ & $\cdots$ \\
  071011 & Yes & $\cdots$ & $\cdots$ & $0.90 \pm 0.20$ & $\cdots$ & $\cdots$ & 
    $1.9 \pm 0.7$ & 0.26 (6) & 0.66 & $\cdots$ \\
  071020 & Yes & $\cdots$ & 2.145 & $0.89 \pm 0.12$ & $\cdots$ & $\cdots$ & 
    $0.58 \pm 0.27$ & 2.16 (14) & 0.52 & $\cdots$ \\
  071122 & Yes & $\cdots$ & 1.14 & $-0.08 \pm 0.09$ & $\cdots$ & $\cdots$ &
    $1.3 \pm 0.6$ & 0.36 (11) & 0.64 & $0.58 \pm 0.05$ \\
  080310 & Yes & $\cdots$ & 2.43 & $0.02 \pm 0.03$ & $0.68_{-0.08}^{+0.11}$ &
    $1.83 \pm 0.02$ & $0.91 \pm 0.10$ & 0.57 (21) & 0.79 & $< 0.14$ \\
  080319A & Yes & $\cdots$ & $\cdots$ & $-0.9 \pm 0.4$ & $0.80 \pm 0.07$ & 
    $0.160_{-0.070}^{+0.136}$ & $2.0 \pm 0.3$ & 1.50 (11) & 0.41 & $\cdots$ \\
  080319B & Yes & $\cdots$ & 0.937 & $1.93_{-0.06}^{+0.04}$ & $1.238 \pm 0.004$ &
    $10.10 \pm 0.17$ & $0.50 \pm 0.02$ & 0.57 (280) & 0.52 & $\cdots$ \\
  080319C & Yes & $\cdots$ & 1.95 & $1.4 \pm 0.2$ & $\cdots$ & $\cdots$ & 
    $2.4 \pm 0.2$ & 2.32 (3) & 0.36 & $0.67 \pm 0.06$ \\
  080320 & Yes & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 
    $\cdots$ & $\cdots$ & $< 0.31$ & $\cdots$ \\
  \enddata
  \tablenotetext{a}{Optical (OT) and Infrared (IRT) transient references:
    GRB\,050607: \citet{GCN.3527}; GRB\,050915A: \citet{GCN.3984};
    GRB\,060923A: \citet{GCN.5587}; GRB\,061222A: \citet{GCN.5975}.}
  \tablenotetext{b}{Redshift references: GRB\,050416A: \citet{snc+07};
    GRB\,050908: \citet{GCN.3948}; GRB\,060210: \citet{GCN.4729};
    GRB\,060502A: \citet{GCN.5052}; GRB\,060510B: \citet{psc+07};
    GRB\,060906: \citet{jfl+06}; GRB\,060908: \citet{GCN.5555};
    GRB\,070208: \citet{GCN.6083}; GRB\,070419A: \citet{GCN.6322};
    GRB\,071003: \citet{plc+08}; GRB\,071020: \citet{GCN.6952};
    GRB\,071122: \citet{GCN.7124}; GRB\,080310: \citet{GCN.7388};
    GRB\,080319B: \citet{GCN.7444}; GRB\,080319C: \citet{GCN.7517}.}
  \tablenotetext{c}{We fitted the flux density to a single or broken
    power-law model of the form $F_{\nu} = t^{-\alpha} \nu^{-\beta}$.}
  \tablenotetext{d}{The optical-to-X-ray spectral index, measured at 
    $t = 10^{3}$\,s.}
  \tablenotetext{e}{We fitted for the host galaxy reddening by fixing the  
    spectral index to $\beta = 0.6$ and assuming an SMC-like extinction law 
    \citep{p92}.}
  \tablenotetext{f}{The optical light curve of GRB\,050820A consists of 
    many power-law segments.  See \citet{ckh+06} for details.}
  \tablenotetext{g}{The optical light curve of GRB\,060906 is not well-described
    by either a single or broken power-law.  The spectral index was calculated
    over only a small period of relatively flat evolution ($t > 10^{4}$\,s).}
\label{tab:early}
\end{deluxetable}
\end{landscape}

